Who's Asking? Investigating Bias Through the Lens of Disability Framed Queries in LLMs

Large Language Models (LLMs) routinely infer users demographic traits from phrasing alone, which can result in biased responses, even when no explicit demographic information is provided. The role of disability cues in shaping these inferences remains largely uncharted. Thus, we present the first systematic audit of disability-conditioned demographic bias across eight state-of-the-art instruction-tuned LLMs ranging from 3B to 72B parameters. Using a balanced template corpus that pairs nine disability categories with six real-world business domains, we prompt each model to predict five demographic attributes - gender, socioeconomic status, education, cultural background, and locality - under both neutral and disability-aware conditions. Across a varied set of prompts, models deliver a definitive demographic guess in up to 97\% of cases, exposing a strong tendency to make arbitrary inferences with no clear justification. Disability context heavily shifts predicted attribute distributions, and domain context can further amplify these deviations. We observe that larger models are simultaneously more sensitive to disability cues and more prone to biased reasoning, indicating that scale alone does not mitigate stereotype amplification. Our findings reveal persistent intersections between ableism and other demographic stereotypes, pinpointing critical blind spots in current alignment strategies. We release our evaluation framework and results to encourage disability-inclusive benchmarking and recommend integrating abstention calibration and counterfactual fine-tuning to curb unwarranted demographic inference. Code and data will be released on acceptance.

==> ICCV2025-Author-Kit-Feb/preamble.tex <==
%
% --- inline annotations
%
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}



==> ICCV2025-Author-Kit-Feb/sec/0_abstract.tex <==
\begin{abstract}
Large Language Models (LLMs) often make implicit assumptions about a user's demographic background such as gender, socioeconomic status, and education level based solely on the phrasing and content of their queries. These assumptions can result in biased responses, even when no explicit demographic information is provided. While such demographic inference has been studied extensively, the role of disability in shaping these inferences remains underexplored.

In this work, we examine how self-declared disability information in user queries influences the demographic assumptions made by state-of-the-art LLMs. We conduct a controlled study across nine disability categories and five core demographic attributes, analyzing both overall response rates and shifts in predicted attribute distributions. Our results show that disability contexts often alter model behavior, reinforcing ableist stereotypes --- for example, linking sensory processing disorders with lower income, or associating learning disabilities with non-Western identities. These effects are further intensified in domain-specific settings such as healthcare and finance.

Our findings underscore the need for intersectional fairness audits that include disability as a key factor, and call for model design choices that reduce overconfident inferences based on user context.
\end{abstract}


==> ICCV2025-Author-Kit-Feb/sec/0_abstract_revised.tex <==
\begin{abstract}
Large Language Models (LLMs) routinely infer users’ demographic traits from phrasing alone, which can result in biased responses, even when no explicit demographic information is provided. The role of disability cues in shaping these inferences remains largely uncharted. Thus, we present the first systematic audit of disability‑conditioned demographic bias across eight state‑of‑the‑art instruction‑tuned LLMs ranging from 3B to 72B parameters. Using a balanced template corpus that pairs nine disability categories with six real‑world business domains, we prompt each model to predict five demographic attributes - gender, socioeconomic status, education, cultural background, and locality - under both neutral and disability‑aware conditions.

Across a varied set of prompts, models deliver a definitive demographic guess in up to 97\% of cases, exposing a strong tendency to make arbitrary inferences with no clear justification. Disability context heavily shifts predicted attribute distributions, and domain context can further amplify these deviations. We observe that larger models are simultaneously more sensitive to disability cues and more prone to biased reasoning, indicating that scale alone does not mitigate stereotype amplification.

Our findings reveal persistent intersections between ableism and other demographic stereotypes, pinpointing critical blind spots in current alignment strategies. We release our evaluation framework and results to encourage disability‑inclusive benchmarking and recommend integrating abstention calibration and counterfactual fine‑tuning to curb unwarranted demographic inference. Code and data will be released on acceptance.
\end{abstract}



==> ICCV2025-Author-Kit-Feb/sec/1_intro.tex <==
\section{Introduction}
\label{sec:intro}

Large Language Models (LLMs) are increasingly deployed in applications that rely on understanding user attributes to personalize experiences, improve accessibility, and deliver targeted support\cite{brown2020languagemodelsfewshotlearners,openai2024gpt4technicalreport,Radford2018ImprovingLU}. However, these models can infer sensitive demographic information such as gender, socioeconomic status, geographic location, and education level from user queries, even when explicit personal identifiers are absent. The presence of specific contexts, such as disability related language, may amplify or alter these inferences, leading to intersectional biases that disproportionately affect marginalized groups~\cite{Caliskan_2017, Gallegos2023BiasAF, Hall2022ASS, Kotek2023GenderBA}.

Recent findings~\cite{cheng2023marked-personas-intersectional,decoding-ableism-intersectional-llm, mitigate-intersectional-diffusion} further show that LLMs frequently associate disability terms with negative sentiment or deficit-oriented frames, thereby amplifying societal stigma. Unlike gender or racial biases - which often have more extensive training data and community-led benchmarking - disability bias remains severely understudied and under-resourced, resulting in amplification patterns that are harder to detect and mitigate. This gap in bias detection infrastructure, coupled with the sparsity of disability-aware corpora, presents unique challenges for fairness in LLMs. As such, understanding how representational and stereotype bias amplification manifests in disability contexts is both a critical and overdue area of inquiry.

Research in bias mitigation has focused primarily on adding guardrails to prevent a model from sharing sensitive information. However, this does not address the root problem, and the inherent biases of the model itself remain, which may affect its perception of the user and be reflected in indirect queries~\cite{yuan2024rigorllmresilientguardrailslarge}. When a model is asked to infer an uncorrelated sensitive attribute from a user prompt, it should refuse to respond as there is insufficient information to make that judgment\cite{yadkori2024mitigatingllmhallucinationsconformal}. However, we show that in many cases, it is likely to respond anyway, reflecting its internal biases.

Understanding how a disability context influences demographic attribute inference is crucial for mitigating risks related to unfair profiling, privacy violations, and reinforcement of societal stereotypes. This work aims to systematically investigate the impact of disability related contexts on LLMs’ demographic inference behaviour to highlight biases, identify model blind spots, and inform ethical AI design and deployment.

%-------------------------------------------------------------------------

The key contributions of this paper are as follows ---
\begin{enumerate}
    \item We demonstrate that LLMs show a noticeable tendency to respond in both a neutral scenario and when a disability is mentioned in the prompt.

    % \item \textbf We show that this tendency to respond has significant variation across different domains 
    
    \item We show that these responses are biased in nature. Further, we show that the biases vary significantly between neutral and various disability scenarios and analyse how model bias changes in the context of various domains and disability types.
    
    % \item \textbf{We show that the model bias is noticeably affected by whether it is a conventionally sensitive attribute.} Attributes like gender and race are conventionally considered sensitive and protections against assumptions on these are well-studied and tested. However, we find that there is a research gap when it comes to less prioritized attributes, such as location or income, leading to strongly biased demographic inference on these across both disability and non-disability scenarios and less representative models.
\end{enumerate}

\section{Background and Related Works}

% TODO: Find relevant papers
% Bias is more of an intro
\subsection{Bias in LLMs}
Large Language Models (LLMs) have demonstrated remarkable performance across a range of NLP tasks; however, they are vulnerable to representational bias and stereotyping. Several studies demonstrate how LLMs absorb and amplify harmful societal biases - especially those tied to gender, race, religion, and health - across both contextual embeddings and generative outputs~\cite{Caliskan_2017, Gallegos2023BiasAF, Kumar2022LanguageGM}. LLMs are proven to reproduce gendered, economic and occupational assumptions, often mirroring imbalances present in training data rather than reflecting equitable or contextually appropriate associations~\cite{Hall2022ASS, Nadeem2020StereoSetMS, Kotek2023GenderBA}. While much of the current literature has centered on the amplification of biases related to gender, race, and political ideology, emerging research sheds light on LLM bias against people with disabilities as well. 

\subsection{Disability bias}
Prior research~\cite{disability-centred-llm-perspectives, impact-disability-fairness-bias, investigating-ableism-mt-conversation} has also shown that models imbibe harmful generalisations and stereotypes about people with disabilities. LLMs tend to associate mentions of disability with perceived negativity~\cite{hassan2021unpacking-ableist-intersectional}. They mirror many prejudices from the training dataset, subtly reinforcing many harmful assumptions about people with disabilities~\cite{disability-centred-llm-perspectives}. These baked-in stereotypes may lead to models discriminating against people who disclose a disability in the hiring process~\cite{impact-disability-fairness-bias}. They also result in overgeneralizations which cause people with disabilities to be misrepresented by these models. Although these are related to our work, they focus on studying disabilities and the prejudice associated with them in isolation. On the other hand, we focus primarily on the cross-study of how disabilities cause models to make biased presumptions about other attributes, such as gender, economic status, and education level.

% TODO: Find relevant papers
\subsection{Hallucinations and abstention} LLMs are known to assume stereotypes and often hallucinate or fabricate facts to justify their assumptions~\cite{Kotek2023GenderBA}.Wan et. al ~\cite{wan2023kellywarmpersonjoseph} introduces the term “hallucination bias”, where LLMs fabricate gendered traits not grounded in input, while Kamruzzaman et al.~\cite{kamruzzaman-etal-2024-investigating} discuss how experiments show that LLMS depict preferential descriptions, with elite Western affiliations being favoured. Previous research has explored ways to combat this through fine-tuning or prompting them to abstain from inferring in cases where there is lack of appropriate context ~\cite{yadkori2024mitigatingllmhallucinationsconformal, madhusudhan2024llmsknowanswerinvestigating}. However, it is noted that  even state-of-the-art LLMs like GPT-4 struggle with abstention, though strategic prompting, such as Chain-of-Thought, can significantly enhance this ability ~\cite{madhusudhan2024llmsknowanswerinvestigating}.

\subsection{Intersectionality of biases}

There has been limited analysis of how the intersection of multiple biases impacts a model’s perception of an individual. Previous works~\cite{cheng2023marked-personas-intersectional, hassan2021unpacking-ableist-intersectional, decoding-ableism-intersectional-llm, intersectional-stereotypes} have primarily examined how LLMs behave when presented with multiple marginalized identities. Notably,~\cite{decoding-ableism-intersectional-llm} focused on how disability interacts with other social categories. In contrast, our work investigates how disability cues lead models to make inferences about unrelated attributes.

Several datasets document harmful stereotypes in intersectional contexts. \cite{cheng2023marked-personas-intersectional} introduced a benchmark to probe identity-based behavior. \cite{intersectional-stereotypes} proposed a dataset capturing stereotype prevalence in three LLMs across intersectional groups. Building on~\cite{cao2022theory, cheng2023marked-personas-intersectional}, it used full-sentence prompts rather than individual words, enabling more complex stereotype analysis.

\cite{hassan2021unpacking-ableist-intersectional} examined ableist bias in BERT using a sentiment analysis task. They showed increased negative sentiment when disability was introduced but found minimal changes under intersectional conditions. Their approach was limited by a narrow verb set and overlapping identity categories. \cite{decoding-ableism-intersectional-llm} studied ableist bias in LLMs across multiple identity combinations using sentiment and social perception metrics. They found that while GPT-4 was less biased than GPT-3.5, bias persisted, especially in intersectional cases.

Some work has explored bias mitigation. \cite{correcting-underrepresentation-intersectional} addressed underrepresentation by inferring dropout rates across identity attributes from small, unbiased samples. \cite{mitigate-intersectional-diffusion} proposed a disentangled attention mechanism to reduce intersectional bias in diffusion models. However, both focus primarily on gender; disability intersections remain underexplored.

A significant limitation in current work in this area is the lack of work on how models perceive the correlation between different attributes or identities. Prior research on intersectional biases primarily served to analyze the biases and stereotypes that were perpetuated at the intersection of disabilities with other attributes, and largely left the correlation between them unstudied. Hence, in this paper, we attempt to analyze how models correlate disabilities with various attributes, such as gender, income, and locality.

\section{Methodology}
 While prior studies have consistently shown that LLMs exhibit systematic biases, including the reinforcement of societal stereotypes and skewed sentiment associations across demographic and occupational domains, this has rarely been examined specifically within the context of accessibility. Thus, this paper analyses the correlation between a model's bias towards people with disabilities and their other attributes, and whether models are more likely to make stereotypical assumptions in the case of people with disabilities.
 
  We do so by by querying the LLM and prompting it to assign gender, economic, educational and cultural attributes to the user\footnote{Please note that many of these, while not truly binary attributes, are presented to the model as binary choices. We make this choice to maintain consistency across attributes and to further demonstrate the tendency of models to make assumptions and perpetuate such prejudices.}, asking this query for both cases where the user is assumed to have no disability and the case where the user is assumed to have a specific disability. We term the percentage of queries to which an LLM responds with a valid option as the response rate. We then compare overall response rates as well as biases towards one label in the attribute over the other.
  
  \subsection{Dataset Selection}
  For our experiments, we use the AccessEval dataset, which consists of paired queries in six real world business domains: Education, Finance, Healthcare, Hospitality, Media, and Technology. The pairs are as follows:

  \begin{itemize}
      \item A \textbf{Neutral Query (NQ)}, which does not reference any disability, and
      \item A corresponding \textbf{Disability Aware Query (DQ)}, which explicitly incorporates disability related context through placeholders for nine disability categories(for systemic evaluation) 
  \end{itemize}

   In this work, we consider the following disability types: Vision impairments, Hearing impairments, Speech impairments, Mobility impairments, Neurological disorders, Genetic and developmental disorders, Learning disorders, Sensory and cognitive disorders, and Mental and behavioral disorders.

  \subsection{Query Formation}
  For the purpose of determining correlations between biases and disability labels, we define five main attributes that we with for the LLM to evaluate the query and assign user labels on: Gender (with label pairs --- male, female), Socioeconomic Status (with label pairs --- Low income, High income), Geographic Location (with label pairs --- Urban, Rural), Educational Background (with label pairs --- Low, High) and Cultural Background(with label pairs --- Western, Non western).
  We then prompt the LLM to determine which label is more apt for the user for each of the five attributes based on the query asked. This is for all ten cases (one with the NQ and one for each of the 9 DQs).

  \subsection{Models}

  Since our aim is to investigate intersectional bias in SOTA LLMs, we chose a representative selection of LLMs covering a variety of sizes and architectures ---
  \begin{itemize}
      \item \textbf{Small ($\sim$3B)} --- Llama-3.2-3B-Instruct~\cite{llama3}, Phi-4-Mini-Instruct~\cite{phi4mini}, and Qwen-2.5-3B-Instruct~\cite{qwen2.5}
      \item \textbf{Medium ($\sim$8B)} --- Llama-3.1-8B-Instruct~\cite{llama3}, Ministral-8B-Instruct~\cite{ministral}, and Qwen-2.5-7B-Instruct~\cite{qwen2.5}
      \item \textbf{Large ($\sim$70B)} --- Llama-3.3-70B-Instruct~\cite{llama3} and Qwen-2.5-72B-Instruct~\cite{qwen2.5}
  \end{itemize}
  
  This selection enables a systematic analysis of how intersectional bias manifests across model scales and architectural design choices, facilitating insights into the dynamics of disability-related intersectional bias in contemporary instruction-tuned LLMs.

  % \subsection{Analysis and Evaluation}
  % We chose to examine the responses generated from the lens of two categories:
  % \begin{itemize}
  %     \item The response rates of the model when prompted to choose between a binary set of options
  %     \item Whether the model displays a strong preference for one label over the other
  % \end{itemize}

  % Based on this, we formulate three more specific research questions. which are as follows:
  % \begin{itemize}
  %     \item RQ1
  %     \item How does a model's response rate vary across both neutral and different disability-aware queries, as well as different fields?
  %     \item Does a model tend to associate certain, disabilities with certain attributes, both with and without the context of different  business domains?     
  % \end{itemize}
  % To evaluate these, we used the following approaches

  
\section{Results and Discussion}
% \subsection{Responsiveness and Inference Bias}
% RQ1
% \subsection{RQ2:What affects Response Rate of LLMs?}
% %\subsection{Response Rates Vs Models, Disability and Domains}
%  % RQ2
% \subsubsection{Which Attributes do LLM are more likely to associate?}
% \subsection{ Influence of Attribute Sensitivity}
% RQ3
% \subsection{Influence of Attribute Sensitivity}
% \subsection{RQ3:}



==> ICCV2025-Author-Kit-Feb/sec/1_intro_revised.tex <==
\section{Introduction}
\label{sec:intro}

Large Language Models (LLMs) are increasingly deployed in applications that rely on understanding user attributes to personalize experiences, improve accessibility, and deliver targeted support~\cite{brown2020languagemodelsfewshotlearners,openai2024gpt4technicalreport,Radford2018ImprovingLU}. However, these models can infer sensitive demographic information such as gender, socioeconomic status, geographic location, and education level from user queries, even when explicit personal identifiers are absent. The presence of specific contexts, such as disability-related language, may amplify or alter these inferences, leading to intersectional biases that disproportionately affect marginalized groups~\cite{Caliskan_2017, Gallegos2023BiasAF, Hall2022ASS, Kotek2023GenderBA, chu2024fairnessllms}.

Recent findings~\cite{cheng2023marked-personas-intersectional,decoding-ableism-intersectional-llm, mitigate-intersectional-diffusion} further show that LLMs frequently associate disability-related terms with negative sentiment or deficit-oriented frames, thereby reinforcing societal stigma. Unlike gender or racial biases - which benefit from more extensive training data and community-led benchmarking - biases related to disability remain markedly underexplored and under-resourced, resulting in amplification patterns that are more difficult to detect and rectify. Critical meta‑analyses suggest that the conceptualization and measurement of bias in NLP systems is often inconsistent and under‑theorized, pointing to the need for more robust fairness frameworks~\cite{blodgett2020languagepower}. This gap in bias detection infrastructure, combined with the scarcity of disability-aware corpora, presents unique challenges for ensuring fairness in LLMs. Accessibility‑focused datasets also remain limited; a recent meta‑analysis highlights continuing issues in demographic representativeness across disability datasets~\cite{gogate2022accessibilitydatasets}. Thus, understanding how representational and stereotype bias amplification manifests in disability contexts is both a critical and overdue area of inquiry.


Most existing research in bias mitigation has focused on adding guardrails to restrict model outputs that include sensitive information~\cite{yuan2024rigorllmresilientguardrailslarge}. However, these safeguards do not address the root problem - the model's internalized biases - which can influence its perceptions of the user and manifest in indirect responses. Ideally, when prompted to infer an uncorrelated sensitive attribute, a model should abstain, as there is insufficient context for such inference~\cite{yadkori2024mitigatingllmhallucinationsconformal}. In practice, however, we find that models frequently respond anyway, revealing latent biases embedded in their training data.

Understanding how disability-related context shapes demographic inference is essential for mitigating risks such as unfair profiling, privacy violations, and the reinforcement of harmful stereotypes. In this paper, we systematically examine the influence of disability cues on LLMs' demographic inference behavior to highlight implicit biases, uncover model blind spots, and inform the development of more equitable AI systems.

%-------------------------------------------------------------------------

The key contributions of this paper are as follows:
% \begin{enumerate}
%     \item We demonstrate that LLMs exhibit a consistent tendency to provide responses in both neutral scenarios and when a disability context is introduced in the prompt.

%     \item We show that these responses reflect systematic biases. Moreover, we analyze how these biases vary across neutral and disability-specific scenarios, revealing distinct shifts based on domain and disability type.
% \end{enumerate}

% \paragraph{Key Contributions.}
\begin{itemize}
    \item \textbf{First prompt-induced demographic inference audit.}  
    We present the earliest large-scale evaluation that measures how disability cues embedded solely in user prompts trigger biased demographic inferences in LLMs.

    \item \textbf{Systematic failure analysis.} we show that across prompts, the eight models guess demographic profiles in up to 97\% of cases; a single disability cue can shift predicted distributions by as much as up to 50\% in some models, exposing prompt-induced stereotype amplification.

    \item \textbf{Comprehensive coverage.}  
    Our audit spans eight instruction-tuned LLMs (3 B–72 B parameters), nine disability categories, six business domains, and five demographic attributes, delivering the most exhaustive intersectional evaluation to date.
\end{itemize}



\section{Background and Related Works}

% TODO: Find relevant papers
% Bias is more of an intro

\subsection{Bias in LLMs}
Large Language Models (LLMs) have demonstrated remarkable performance across a wide range of NLP tasks; however, they remain susceptible to representational bias and stereotyping. Prior research has shown that LLMs often absorb and reproduce harmful societal biases - especially those tied to spoken language~\cite{agarwal2025aligningllmsmultilingualconsistency}, gender~\cite{panda2025daiqauditingdemographicattribute}, race, religion, and health - across both contextual embeddings and generative outputs~\cite{cahyawijaya-etal-2025-crowdsource, meghwani-etal-2025-hard, Gallegos2023BiasAF, Kumar2022LanguageGM,agarwal-etal-2025-mvtamperbench,pattnayak2025hybrid}. These models frequently reflect the imbalances present in their training data, reproducing gendered, socioeconomic, and occupational assumptions rather than equitable or contextually informed representations~\cite{Hall2022ASS, Nadeem2020StereoSetMS, Kotek2023GenderBA, patel2025sweeval}. While substantial literature exists on bias amplification related to gender, race, and political ideology, research into ableist bias in LLMs - bias against people with disabilities - is only beginning to gain scholarly traction.

\subsection{Disability bias}
Emerging studies~\cite{disability-centred-llm-perspectives, investigating-ableism-mt-conversation} reveal that LLMs often encode and reflect deeply entrenched stereotypes about people with disabilities. For instance, models tend to associate disability-related terms with negative sentiment~\cite{hassan2021unpacking-ableist-intersectional}, echoing societal stigma found in training data. These encoded assumptions are not merely superficial - they can meaningfully shape the outputs of LLMs, resulting in misrepresentations or even algorithmic discrimination. This is particularly concerning in high-stakes contexts like hiring~\cite{impact-disability-fairness-bias}, where disclosure of a disability can lead to skewed responses. While prior work has largely focused on disability bias in isolation, our study probes a more nuanced intersectional space: how disability contexts influence inferences about seemingly unrelated demographic attributes such as gender, income level, and educational background.

\subsection{Hallucinations and abstention}
LLMs are also known to fabricate details or exaggerate associations - particularly when making inferences from sparse input. This phenomenon, known as "hallucination bias," occurs when models generate unsupported demographic traits or correlations~\cite{Kotek2023GenderBA, wan2023kellywarmpersonjoseph}. For instance, Kamruzzaman et al.~\cite{kamruzzaman-etal-2024-investigating} found that models disproportionately favored elite Western affiliations in synthesized content, even when prompts were neutral. Recent work has advocated fine-tuning and strategic prompting (e.g., Chain-of-Thought) to encourage abstention when contextual grounding is lacking~\cite{yadkori2024mitigatingllmhallucinationsconformal, madhusudhan2024llmsknowanswerinvestigating}. Yet, even advanced models like GPT-4 have been shown to struggle with abstention - particularly in subtle or intersectional cases where demographic inferences appear plausible.

\subsection{Intersectionality of biases}
There remains limited but growing attention on how intersecting identities influence LLM behavior. While several recent works~\cite{cheng2023marked-personas-intersectional, hassan2021unpacking-ableist-intersectional, decoding-ableism-intersectional-llm, intersectional-stereotypes,agarwal2025rciscoreevaluatingglobal,patel2025pcrimeasuringcontextrobustness} have evaluated how multiple marginalized identities interact within prompts and input space, few studies have examined how disability cues lead to inferred biases about unrelated attributes. Notably,~\cite{decoding-ableism-intersectional-llm} explored ableist bias in tandem with other identity categories, using sentiment and social perception metrics. In contrast, our study isolates how disability acts as a contextual modifier for demographic assumptions.

To support such analysis, various benchmark datasets have emerged. For instance,~\cite{cheng2023marked-personas-intersectional} introduced a probing framework for identity-based behavior using persona-based prompts, while~\cite{intersectional-stereotypes} presented a stereotype prevalence dataset for intersectional identities across LLMs. These newer datasets emphasize richer, sentence-level stimuli that better reflect real-world complexity~\cite{cao2022theory,dua2025flexdocparameterizedsamplingdiverse}.

Earlier sentiment-based evaluations~\cite{hassan2021unpacking-ableist-intersectional} using BERT found that disability-related prompts consistently triggered more negative sentiment. However, changes under intersectional conditions were modest - partly due to dataset limitations such as overlapping identity labels. More recent work~\cite{decoding-ableism-intersectional-llm} has highlighted that even large-scale models like GPT-4 retain measurable bias under intersectional prompts, despite appearing less biased than earlier versions.

On the mitigation front, work such as~\cite{correcting-underrepresentation-intersectional} has sought to improve fairness by inferring dropout patterns from unbiased samples, while others~\cite{mitigate-intersectional-diffusion} have proposed architectural interventions like disentangled attention mechanisms. Still, the majority of these efforts focus on gender bias, with disability-related intersections remaining underexplored.

A significant and underexamined aspect of this space is how LLMs correlate different identity markers. Most prior work has evaluated whether bias exists, not how assumptions about one attribute (e.g., disability) trigger biased predictions about another (e.g., income or gender). Our work addresses this gap by directly analyzing the correlational inferences made by models when disability-related context is introduced into queries.


\section{Methodology}

While prior studies have consistently shown that LLMs exhibit systematic biases - including the reinforcement of societal stereotypes and skewed sentiment associations across demographic and occupational domains - these patterns have rarely been examined through the lens of accessibility. This paper aims to bridge that gap by analyzing whether the presence of disability-related context affects how models infer other demographic attributes, and whether such contexts make models more prone to stereotypical assumptions about the user.

To investigate this, we query state-of-the-art LLMs and prompt them to infer gender, socioeconomic status, educational attainment, cultural background, and geographic location for a hypothetical user\footnote{While these are not inherently binary attributes, we frame them as binary choices to ensure consistency across queries and to more clearly reveal the models' propensity to default to normative or stereotypical responses.}. We do this across two conditions: (i) where the query contains no disability context (neutral) and (ii) where it includes a specific disability context. We define the \textbf{response rate} as the percentage of queries for which an LLM produces a definitive inference rather than refusing with a canned response. We then compare overall response rates and analyze directional biases across the attribute labels.

\subsection{Dataset Selection}
For our experiments, we use the AccessEval dataset~\cite{AccessEvalDataset,panda2025accessevalbenchmarkingdisabilitybias}, which comprises sets of queries spanning six real-world business domains: Education, Finance, Healthcare, Hospitality, Media, and Technology. Each set consists of:

\begin{itemize}
    \item A \textbf{Neutral Query (NQ)} that contains no mention of disability, and
    \item A corresponding set of \textbf{Disability-Aware Queries (DQs)} that explicitly introduces disability-related context using placeholders representing nine disability categories (used for systematic evaluation).
\end{itemize}

Our study includes the following disability types: Vision impairments, Hearing impairments, Speech impairments, Mobility impairments, Neurological disorders, Genetic and developmental disorders, Learning disorders, Sensory and cognitive disorders, and Mental and behavioral disorders.

\subsection{Query Formation}

\begin{table}[t]
  \centering
  \resizebox{\linewidth}{!}{%
    \begin{tabular}{@{}p{0.24\linewidth}p{0.76\linewidth}@{}}
      \toprule
      \textbf{Prompt} &
      You will be given a question in text form.  
      Your task is to infer the author’s demographics by selecting \emph{one} option per category below  
      and return the result in the exact JSON schema (include the original question under the key \textit{"query"}).
      
      \textit{\{actual\_query\}}\\[4pt]
    \midrule
      \textbf{Categories} &
      Age: \{Child, Adult\}\\
      & Gender: \{Male, Female\}\\
      & Socioeconomic Status: \{Low income, High income\}\\
      & Geographic Location: \{Urban, Rural\}\\
      & Educational Background: \{Low, High\}\\
      & Cultural Background: \{Western, Non-western\}\\[4pt]

    \midrule
      \textbf{Question} & \textit{actual\_query}, selected from the dataset\\
      \bottomrule
    \end{tabular}%
  }
  \caption{Instruction prompt supplied to the LLM for demographic inference.}
  \vspace{-1em}
  \label{tab:prompt}
\end{table}

To measure the correlation between disability context and inferred user attributes, we define five core demographic dimensions: Gender (\textit{male, female}), Socioeconomic Status (\textit{low income, high income}), Geographic Location (\textit{urban, rural}), Educational Background (\textit{low, high}), and Cultural Background (\textit{Western, Non-Western}). 

For each of these five attributes, we prompt the model to infer the most plausible label based solely on the phrasing of the user query. Details of the prompt are provided in Table~\ref{tab:prompt} This process is repeated for all ten conditions - one for the NQ and one each for the nine DQs - providing a comprehensive view of how disability contexts affect demographic inferences.

\subsection{Models}

To systematically analyze intersectional bias, we evaluate a representative range of instruction-tuned LLMs across three model scales:

\begin{itemize}
    \item \textbf{Small ($\sim$3B)} - Llama 3.2 3B Instruct~\cite{llama3}, Phi 4 Mini Instruct~\cite{phi4mini}, and Qwen 2.5 3B Instruct~\cite{qwen2.5}
    \item \textbf{Medium ($\sim$8B)} - Llama 3.1 8B Instruct~\cite{llama3}, Ministral 8B Instruct~\cite{ministral}, and Qwen 2.5 7B Instruct~\cite{qwen2.5}
    \item \textbf{Large ($\sim$70B)} - Llama 3.3 70B Instruct~\cite{llama3} and Qwen 2.5 72B Instruct~\cite{qwen2.5}
\end{itemize}

This range enables robust comparison across architectures and parameter scales, offering insight into whether larger or differently structured models exhibit more or less disability-related intersectional bias in response behavior. We selected these models based on their open-source nature, which ensures transparency, accessibility, and reproducibility of our methodology and findings.

  % \subsection{Analysis and Evaluation}
  % We chose to examine the responses generated from the lens of two categories:
  % \begin{itemize}
  %     \item The response rates of the model when prompted to choose between a binary set of options
  %     \item Whether the model displays a strong preference for one label over the other
  % \end{itemize}

  % Based on this, we formulate three more specific research questions. which are as follows:
  % \begin{itemize}
  %     \item RQ1
  %     \item How does a model's response rate vary across both neutral and different disability-aware queries, as well as different fields?
  %     \item Does a model tend to associate certain, disabilities with certain attributes, both with and without the context of different  business domains?     
  % \end{itemize}
  % To evaluate these, we used the following approaches

  
\section{Results and Discussion}
% \subsection{Responsiveness and Inference Bias}
% RQ1
% \subsection{RQ2:What affects Response Rate of LLMs?}
% %\subsection{Response Rates Vs Models, Disability and Domains}
%  % RQ2
% \subsubsection{Which Attributes do LLM are more likely to associate?}
% \subsection{ Influence of Attribute Sensitivity}
% RQ3
% \subsection{Influence of Attribute Sensitivity}
% \subsection{RQ3:}



==> ICCV2025-Author-Kit-Feb/sec/2_formatting.tex <==
\section{Formatting your paper}
\label{sec:formatting}

All text must be in a two-column format.
The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
Columns are to be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
The second and following pages should begin 1 inch (2.54 cm) from the top edge.
On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
high.
%
Page numbers should be in the footer, centered and $\frac{3}{4}$ inches from the bottom of the page.
The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
The \LaTeX\ template takes care of this when used properly.



%-------------------------------------------------------------------------
\subsection{Type style and fonts}

Wherever Times is specified, Times Roman may also be used.
If neither is available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE.
Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
Leave two blank lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type.
This information is to be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT.
Type main text in 10-point Times, single-spaced.
Do NOT use double-spacing.
All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
Make sure your text is fully justified---that is, flush left and flush right.
Please do not place any additional blank lines between paragraphs.

Figure and table captions should be 9-point Roman type as in \cref{fig:onecol,fig:short}.
Short captions should be centred.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

FIRST-ORDER HEADINGS.
(For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before, and one blank line after.

SECOND-ORDER HEADINGS.
(For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before, and one after.
If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use footnotes\footnote{This is what a footnote looks like.
It often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{Cross-references}

For the benefit of author(s) and readers, please use the
{\small\begin{verbatim}
  \cref{...}
\end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross-reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, please see \cref{fig:onecol} and \cref{tab:example}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
  You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
\end{quotation}
If you do not wish to abbreviate the label, for example at the beginning of the sentence, you can use the
{\small\begin{verbatim}
  \Cref{...}
\end{verbatim}}
command. Here is an example:
\begin{quotation}
  \Cref{fig:onecol} is also quite important.
\end{quotation}

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
When referenced in the text, enclose the citation number in square brackets, for
example~\cite{Authors14}.
Where appropriate, include page numbers and the name(s) of editors of referenced books.
When you cite multiple papers at once, please make sure that you cite them in numerical order like this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
If you use the template as advised, this will be taken care of automatically.

\begin{table}
  \centering
  \begin{tabular}{@{}lc@{}}
    \toprule
    Method & Frobnability \\
    \midrule
    Theirs & Frumpy \\
    Yours & Frobbly \\
    Ours & Makes one's heart Frob\\
    \bottomrule
  \end{tabular}
  \caption{Results.   Ours is better.}
  \label{tab:example}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
Instead use
{\small\begin{verbatim}
  \centering
\end{verbatim}}
at the beginning of your figure.
Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it's almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
Hence avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.

==> ICCV2025-Author-Kit-Feb/sec/3_finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.

==> ICCV2025-Author-Kit-Feb/sec/RQ_1.tex <==
% \subsection{Responsiveness and Inference Bias}
\subsection{Do LLMs respond to Biased Attributes?}

\begin{figure*}
  \centering
  \begin{subfigure}{0.49\linewidth}
    \includegraphics[width=\textwidth]{ICCV2025-Author-Kit-Feb/fig/rq1_neutral.png}
    \caption{Average response rate across attributes on neutral queries.}
    \label{fig:short-a}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.49\linewidth}
    \includegraphics[width=\linewidth]{ICCV2025-Author-Kit-Feb/fig/rq1_disability.png}
    \caption{Average response rate across attributes on disability queries.}
  \end{subfigure}
  \caption{Comparison of the response rate of models on neutral and average of disability queries. Models with the same color have similar parameter counts.}
  \label{fig:rq1-response-rate}
\end{figure*}

As seen in Figure~\ref{fig:rq1-response-rate}, the average response rate in the neutral scenario averaged across all attributes is 58.6\%, with significant variation between models. Phi-4 shows the lowest response bias i.e. highest abstention rate on average compared to all other models. This remains consistent in both disability and non-disability contexts. It has a response rate of 15\% in the neutral scenario and 13\% on average across disabilities. Qwen 72B, on the other hand, has the highest response rate, barely abstaining from answering queries in either scenario. It has a response rate of 97\% in a disability context and 94\% in a neutral context. We see that overall, the response rate remains relatively unchanged both in the neutral scenario and in the average disability scenario, with a maximum change of 4\% displayed by Qwen 7B. The only exception to this is Llama 3.3 with an increase of 12\% response rate in the average disability scenario. There is an overall average increase of 1.5\% on disability queries as compared to neutral queries, however, this is primarily driven by the outlier increase in Llama 3.3. Excluding Llama 3.3, the average increase or decrease in response rates in the disability scenario is 0\%.

Hence, we see that the presence or absence of a disability, on average, \textbf{does not have any noticeable effect} on the response rate of a model. This also shows the limitations of current techniques in the context of abstaining from answering sensitive queries, especially when it comes to disabilities.

\begin{table}
  \centering
  \resizebox{\linewidth}{!}{%
    \begin{tabular}{@{}lcc@{}}
      \toprule
      Model Size & Neutral Scenario (\%) & Disability Scenario (\%) \\
      \midrule
      Small (3--3.8B) & 48.9 & 49.1 \\
      Medium (7--8B) & 53.7 & 53.3 \\
      Large (70B+) & 81.9 & 89.9 \\
      \bottomrule
    \end{tabular}%
  }
  \caption{Average response rates by model size in neutral and disability scenarios.}
  \label{tab:response-rates}
\end{table}

We also observe in table~\ref{tab:response-rates} that increasing model size also \textbf{increases its response rate.} Previous works have shown that larger models are seen to have better performance by both qualitative and quantitative metrics, but we observe that this is not the case with response bias. Response bias remains prevalent in larger models. As the table shows, the average response rate of models having on the order of 70B parameters is 81.9\% in the neutral scenario and 89.9\% in the disability scenario, whereas that of small models is only 48.9\% in the neutral scenario and 49.1\% in the disability scenario. This suggests that while larger models are better at generating fluent and relevant responses, they may also be less cautious, making them more likely to answer biased or inappropriate questions unless stronger safety measures are in place.

\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{ICCV2025-Author-Kit-Feb/fig/rq1_radar.png}
  \caption{Average response rate for each attribute on neutral queries.}
  \label{fig:rq1-radar}
\end{figure}

%% TODO: DO WE ADD DISABILITY RADAR? OR MENTION IN SUPPLEMENTARY?

As we observed in figure~\ref{fig:rq1-response-rate}, response rate is not significantly impacted by presence or absence of a disability. It is also not affected by the specific disability type, as we discuss in our supplementary material. However, figure~\ref{fig:rq1-radar} shows that attributes have a very noticeable impact on the response rate. Further, the response graphs vary visibly between models. For instance, the 70B models tend to respond to all questions equally regardless of attribute. Ministral primarily responds only to questions on education, at a response rate of 90.2\%, while Llama 3.2 3B responds relatively evenly to all queries except gender, where it strongly abstains. We observe that economic status has the lowest response rate across models on average of 40.3\%, closely followed by gender at 43.8\%. Meanwhile, education has by far the highest response rate of 71.7\%. These findings suggest that models are not uniformly sensitive to demographic attributes, as certain topics like education prompt high response rates, while others like gender or economic status elicit more caution or uncertainty. This uneven responsiveness hints at implicit prioritizations during training, in terms of which attributes are considered sensitive and how safety behaviors are calibrated.

==> ICCV2025-Author-Kit-Feb/sec/RQ_1_revised.tex <==
% \subsection{Responsiveness and Inference Bias}
\subsection{Do LLMs respond to Biased Attributes?}

\begin{figure*}
  \centering
  \begin{subfigure}{0.49\linewidth}
    \includegraphics[width=\textwidth]{ICCV2025-Author-Kit-Feb/fig/rq1_neutral.png}
    \caption{Average response rate across attributes on neutral queries.}
    \label{fig:short-a}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.49\linewidth}
    \includegraphics[width=\linewidth]{ICCV2025-Author-Kit-Feb/fig/rq1_disability.png}
    \caption{Average response rate across attributes on disability queries.}
  \end{subfigure}
  \caption{Overall response rate of eight instruction-tuned LLMs averaged across attributes. Bars represent average response rate, the mean percentage of prompts answered with a definitive response for (a) neutral and (b) disability-framed queries. Colors group models by parameter scale.}
  \vspace{-1em}
  \label{fig:rq1-response-rate}
\end{figure*}


As shown in Figure~\ref{fig:rq1-response-rate}, the average response rate in the neutral scenario across all attributes is 58.6\%, though this varies significantly by model. Among them, Phi 4 demonstrates the strongest abstention behavior (i.e., lowest response rate), with 15\% response rate in the neutral scenario and 13\% on average in disability contexts - indicating strong caution in drawing inferences. In contrast, Qwen 72B has the highest response rate, answering 94\% of neutral queries and 97\% of disability-related queries, suggesting a minimal threshold for abstention.

Overall, the presence of disability-related context does not substantially affect model response rates. Most models show marginal variation (within a 4\% range), with the exception of Llama 3.3, which exhibits a 12\% increase in response rate for disability scenarios. Without this outlier, the net difference between neutral and disability scenarios across models rounds to approximately 0\%. This suggests that current instruction-tuned LLMs do not generally adjust their willingness to answer based on the inclusion of disability information.

These findings raise important questions about the robustness of abstention mechanisms in LLMs. Although prior research emphasizes the importance of abstaining from speculative demographic inference in low-context settings, our results indicate that models do not treat disability cues as particularly sensitive. This points to a gap in how abstention behaviors are calibrated in the presence of disability language, a concern that has implications for fairness and privacy preservation.

\begin{table}[t]
  \centering
  \resizebox{\linewidth}{!}{%
    \begin{tabular}{@{}lcc@{}}
      \toprule
      Model Size & Neutral Scenario (\%) & Disability Scenario (\%) \\
      \midrule
      Small (3--3.8B) & 48.9 & 49.1 \\
      Medium (7--8B) & 53.7 & 53.3 \\
      Large (70B+) & 81.9 & 89.9 \\
      \bottomrule
    \end{tabular}%
  }
  \caption{Average response rates by model size in neutral and disability scenarios.}
  \vspace{-1em}
  \label{tab:response-rates}
\end{table}

As shown in Table~\ref{tab:response-rates}, larger models are substantially more likely to respond to attribute inference prompts. Models in the 70B+ range exhibit response rates near 90\% even in disability contexts, compared to under 50\% for small models. This indicates a correlation between model size and the propensity to produce definitive, and potentially biased, outputs.

This size-related increase in responsiveness may stem from training scale, increased capacity to generalize, or overconfidence in low-context settings. However, high response rates do not necessarily reflect appropriate behavior - particularly in cases where the prompt does not provide sufficient context for a grounded inference. Without well-calibrated abstention or confidence mechanisms, larger models may amplify stereotype risks by generating unwarranted demographic assumptions.

\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{ICCV2025-Author-Kit-Feb/fig/rq1_radar.png}
  \caption{Attribute-wise response rate on neutral queries. Represents, for each model, the proportion of queries answered across demographic attributes, highlighting lower willingness to answer on income and gender.}
  \label{fig:rq1-radar}
  % \vspace{-1em}
\end{figure}

Figure~\ref{fig:rq1-radar} highlights that attribute type - not just model architecture - significantly influences response behavior. While model response rates to education-related questions are highest (averaging 71.7\%), questions related to economic status (40.3\%) and gender (43.8\%) see low response rates. This suggests that models may have been fine-tuned to be more cautious in areas considered socially sensitive.

Interestingly, model behaviors also diverge in attribute-specific ways. For example, the Ministral model demonstrates high responsiveness to educational prompts (90.2\%) but abstains from most others. Llama 3.2 3B, in contrast, abstains heavily on gender while responding more evenly across other categories. These disparities reflect implicit value judgments embedded in training or alignment strategies - indicating that models treat certain attributes as more "answerable" than others.



==> ICCV2025-Author-Kit-Feb/sec/RQ_2.tex <==
\subsubsection{Response Rate by Disability Type}

\begin{figure}[h]
  \centering
  \includegraphics[width=\linewidth]{ICCV2025-Author-Kit-Feb/fig/rq2.1_avg.png}
  \caption{Average response rate for each disability type mentioned in the query. Neutral represents no disability mentioned.}
  \label{fig:rq2.1-avg}
\end{figure}

Figure~\ref{fig:rq2.1-avg} shows the average response rate for each model across disability types. While the overall response rate is relatively stable within each model, subtle but consistent differences emerge across specific attributes. Notably, as observed earlier, models tend to respond at almost equal rates whether the query contains a mention of disability or not, with a slight change in response rate observed for certain disability-related queries. 

Small models show more noticeable trends in terms of having greater variance in response rates based on disability type. For instance, Qwen 7B responds at a noticeably higher rate to queries where genetic and developmental disorders are mentioned. In contrast, larger models like Llama 3.3 70B and Mistral 8B maintain higher and more consistent response rates across all categories. We also notice a visible difference between model families, with all three Llama models generally having a response rate over 70\%, while in the Qwen model family, only the largest model, 72B, shows a response rate above 40\%. This trend is observed across disability types.

This suggests that model size and architecture all play a role in robustness to disability-related prompts, potentially reflecting differences in training scale, alignment strategies, or exposure to diverse linguistic representations of disability.

==> ICCV2025-Author-Kit-Feb/sec/RQ_2_revised.tex <==
% \subsubsection{Response Rate by Disability Type}

\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{ICCV2025-Author-Kit-Feb/fig/rq2.1_avg.png}
  \caption{Response rate by disability category. Average fraction of answered prompts for nine disability types compared with the neutral baseline, showing that disability context only marginally affects models’ willingness to respond.}
  \vspace{-1em}
  \label{fig:rq2.1-avg}
\end{figure}

Figure~\ref{fig:rq2.1-avg} illustrates the average response rate by disability type across models. While each model’s overall response rate remains relatively stable, subtle yet consistent differences emerge based on the specific disability mentioned in the prompt. As previously noted, most models maintain comparable response rates between neutral and disability contexts, suggesting that disability alone does not systematically alter response behavior.

However, more nuanced patterns appear when disaggregating by disability type. Smaller models display greater variability in response rates depending on the specific disability referenced. For example, Qwen 7B exhibits a pronounced increase in responsiveness to prompts mentioning genetic and developmental disorders. In contrast, larger models such as Llama 3.3 70B and Ministral 8B Instruct maintain both high and stable response rates across all disability types.

Differences are also apparent across model families. The Llama models generally respond at rates above 70\% for all disability types, demonstrating a consistent pattern regardless of the specific condition. In contrast, within the Qwen family, only the 72B model achieves a response rate exceeding 40\%, with smaller variants exhibiting much lower rates. These disparities suggest that both scale and architectural design significantly influence how models engage with disability-related prompts.

These trends may be reflective of model-specific exposure to diverse linguistic representations of disability or differing alignment strategies used during instruction tuning. Importantly, the tendency of smaller models to fluctuate more across disability types could signal instability in sensitivity calibration - raising concerns about inconsistent behavior when handling different disability categories.



==> ICCV2025-Author-Kit-Feb/sec/RQ_3.tex <==
\subsection{LLM bias in a disability scenario}
% RQ3.1 Figures
\begin{figure*}
\centering
  \begin{subfigure}{0.49\linewidth}
    \includegraphics[width=\textwidth]{fig/rq3/rq3.1_gender.png}
    \caption{Gender}
    \label{fig:rq3.1-attributes-gender}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.49\linewidth}
    \includegraphics[width=\textwidth]{fig/rq3/rq3.1_income.png}
    \caption{Income}
    \label{fig:rq3.1-attributes-income}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.49\linewidth}
    \includegraphics[width=\textwidth]{fig/rq3/rq3.1_western.png}
    \caption{Culture}
    \label{fig:rq3.1-attributes-culture}
  \end{subfigure}

  \vspace{0.5em}

  \begin{subfigure}{0.49\linewidth}
    \includegraphics[width=\textwidth]{fig/rq3/rq3.1_locality.png}
    \caption{Locality}
    \label{fig:rq3.1-attributes-locality}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.49\linewidth}
    \includegraphics[width=\textwidth]{fig/rq3/rq3.1_education.png}
    \caption{Education}
    \label{fig:rq3.1-attributes-education}
  \end{subfigure}

  \caption{Model bias by attribute for various disability types. Note the significant variations in bias based on disability type.}
  \label{fig:rq3.1-attributes}
\end{figure*}

% RQ3.2 Figures
\begin{figure*}
\centering
  \begin{subfigure}{0.49\linewidth}
    \includegraphics[width=\textwidth]{fig/rq3/rq3.2_gender.png}
    \caption{Gender}
    \label{fig:rq3.2-attributes-gender}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.49\linewidth}
    \includegraphics[width=\textwidth]{fig/rq3/rq3.2_income.png}
    \caption{Income}
    \label{fig:rq3.2-attributes-income}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.49\linewidth}
    \includegraphics[width=\textwidth]{fig/rq3/rq3.2_western.png}
    \caption{Culture}
    \label{fig:rq3.2-attributes-culture}
  \end{subfigure}

  \vspace{0.5em}

  \begin{subfigure}{0.49\linewidth}
    \includegraphics[width=\textwidth]{fig/rq3/rq3.2_locality.png}
    \caption{Locality}
    \label{fig:rq3.2-attributes-locality}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.49\linewidth}
    \includegraphics[width=\textwidth]{fig/rq3/rq3.2_education.png}
    \caption{Education}
    \label{fig:rq3.2-attributes-education}
  \end{subfigure}

  \caption{Model biases by attribute for different question domains. Notice the variance in bias across domains.}
  \label{fig:rq3.2-attributes}
\end{figure*}
As visible in figure~\ref{fig:rq3.1-attributes-gender}, there is a general male bias irrespective of the existence or type of disability though not nearly as strong a preference as is there in other attribute pairs. However, it is also visible that there is a significant variance in model responses, based on both the mention of a disability, as well as the type of disability mentioned. The models depict a strong tendency to associate neutrality (lack of disabilities) with the male gender. Addtionally there was a smaller, but still noticeable spike in assumptions of male gender in the case of learning disorders, neurological disorders and speech impairments. Conversely, while disabilities in general are clearly associated with the female gender there is a distinct spike when it comes to sensory and cognitive disorders. The model's consistent association of male gender with “no disability” aligns with the sociological concept of male default normativity. The spike toward male gender predictions for learning disorders, neurological disorders, and speech impairments may reflect gendered health biases that perceive such disabilities as more typical in boys (e.g., ADHD, autism)—consistent with psychological research showing higher male diagnosis rates and stronger stereotypes linking neurological differences with males, while the overall trend reflects an intersectional stereotype: linking disability with dependence/vulnerability, and further associating that with femininity.

Another interesting observation is made with respect to the responses of models with respect to model size. While LLama moves from a strong female bias towards people with disabilities towards an almost 50-50 response (demonstrating possible randomisation in larger models) with an increase in model size, Qwen 3B has a low response rate and an almost 100\% male bias while Qwen 72 B has a much higher response rate and has an almost 100 percent female response rate.

With respect to~\ref{fig:rq3.1-attributes-income}, all models except LLama 3B depict a strong general bias toward predicting a higher economical class. This is further exacerbated in the case of NQs, leading us to assume that it associates disabilities in general with lower income classes. Due to this, there is less of a trend seen in models with respect to individual disability types with respect to economic status, especially since the models tend to predict high income irrespective of whether a disability is present in the query. The models do, however, show relative associations of low income responses with mobility impairments, genetic and developmental disorders, mental health and behavioral disorders, and speech impairments. Models with lower response rates also demonstrate relatively higher association of lower income with sensory and cognitive disabilities. However, models are much less likely to associate neurological disorders and hearing disorders with lower income. The relative association of certain disability types with poverty reflects real-world ableist economic stereotypes, where visible or developmental disabilities are linked to dependence or reduced opportunity. Some disability types like hearing loss or neurological conditions escape this association, reflecting asymmetric bias and underscoring how models may absorb cultural myths around "competent" versus "dependent" disabilities.

In the case of attributes regarding Culture, Educational Levels and Localities, the model overwhelmingly assumes the association of any query irrespective of disability with Western, Urban and  High Education as observed in figures~\ref{fig:rq3.1-attributes-culture}, \ref{fig:rq3.1-attributes-education}, and \ref{fig:rq3.1-attributes-locality}. This is demonstrates the models' bias, as well as their willingness to assume one label over the other in attributes that are not traditionally considered sensitive. In the case of Culture (\ref{fig:rq3.1-attributes-culture}), we can see that Ministral 8B and Qwen 2.5 3B tend to relatively associate Genetic and Developmental Disorders, Mobility Impairments and Sensory and Cognitive Disorders with non-western communities. Additionally, they also associate almost 100\% of neutral queries with western communities. However due to the highly skewed nature of the results, commenting on this in an accessibility context becomes difficult.

 In the case of Locality (\ref{fig:rq3.1-attributes-locality}), the models assume that the user is from an urban region with almost 100\% likelihood, thus making disability-specific investigations irrelevant. The models' responses in the case of Education(\ref{fig:rq3.1-attributes-education}) appear to be more significant, with almost all models having a near 100\% likelihood of assuming high education in the case of neutral queries. Learning disabilities and Genetic and Developmental disorders on the other hand, seem to have a relative dip, pointing to their relative association with lower education. The models also tend to assume a stronger likelihood of Sensory and Cognitive disabilities in highly educated people. However, the overall symmetry of the graph points to the net bias of the model towards higher education outweighing any disability specific bias.

 The existence of a general trend among models enables us to examine the overall behaviour displayed with respect to each disability. Another way we examine it is through the lens of business domains. 

 Figure (\ref{fig:rq3.2-attributes}) depicts that the models tend to show common spikes with respect to business domains, irrespective of the presence of a disorder or the specific type of disorder mentioned. In the case of Gender(\ref{fig:rq3.2-attributes-gender}), All NQs and DQs show a distinct association of the male gender with Technology, Healthcare and Finance, while strongly associating Education and Hospitality with the female Gender.

 In the case of Income(\ref{fig:rq3.2-attributes-income}) the models respond with 'low income less than 20 \% of the time in the case of every business domain except Finance, where the percent of low income responses doubles. 
 
  In the case of Culture(\ref{fig:rq3.2-attributes-culture}) and Locality(\ref{fig:rq3.2-attributes-locality}) the models respond with western, and urban respectively nearly 100\% of the time displaying a common bias irrespective of disability or business domain. In the case  of Education Level(\ref{fig:rq3.2-attributes-education}) the graph is almost symmetrical, although models do notably assume a lower education level for questions posed by people with learning disabilities in finance. However the overall symmetry in the graph tends to represent a net bias towards answers that assume every user has a high education level.

  All in all, it is clear that domain specific biases have a tendency to influence model answers more than disability specific biases, though the strength of association varies based on the existence of a disability and the disability type in a manner similar to that discussed in figure (\ref{fig:rq3.1-attributes}).

==> ICCV2025-Author-Kit-Feb/sec/RQ_3_revised.tex <==
\subsection{How do disability cues shape demographic bias in LLMs?
}
% RQ3.1 Figures
\begin{figure*}
\centering
  \begin{subfigure}{0.49\linewidth}
    \includegraphics[width=\textwidth]{fig/rq3/rq3.1_gender.png}
    \caption{Gender (\% male)}
    \label{fig:rq3.1-attributes-gender}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.49\linewidth}
    \includegraphics[width=\textwidth]{fig/rq3/rq3.1_income.png}
    \caption{Socioeconomic status (\% low income)}
    \label{fig:rq3.1-attributes-income}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.49\linewidth}
    \includegraphics[width=\textwidth]{fig/rq3/rq3.1_western.png}
    \caption{Cultural background (\% non-Western)}
    \label{fig:rq3.1-attributes-culture}
  \end{subfigure}

  \vspace{0.5em}

  \begin{subfigure}{0.49\linewidth}
    \includegraphics[width=\textwidth]{fig/rq3/rq3.1_locality.png}
    \caption{Geographical locality (\% local)}
    \label{fig:rq3.1-attributes-locality}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.49\linewidth}
    \includegraphics[width=\textwidth]{fig/rq3/rq3.1_education.png}
    \caption{Educational background (\% high education)}
    \label{fig:rq3.1-attributes-education}
  \end{subfigure}

  \caption{\textbf{Bias by disability type.}
For each of nine disability categories, the plot reports the proportion of answers in which eight instruction-tuned LLMs select the \emph{first} label of a demographic pair.  
Separate panels show the share of predictions labelled \textit{male}, \textit{low income}, \textit{non-Western}, \textit{local} and \textit{high education}.  
Marked shifts - for example, a stronger low income bias for Genetic and Developmental disorders displayed by Ministral - highlight how specific disabilities amplify particular stereotypes.}
\vspace{-1em}
  \label{fig:rq3.1-attributes}
\end{figure*}

% RQ3.2 Figures
\begin{figure*}
\centering
  \begin{subfigure}{0.49\linewidth}
    \includegraphics[width=\textwidth]{fig/rq3/rq3.2_gender.png}
    \caption{Gender (\% male)}
    \label{fig:rq3.2-attributes-gender}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.49\linewidth}
    \includegraphics[width=\textwidth]{fig/rq3/rq3.2_income.png}
    \caption{Socioeconomic status (\% low income)}
    \label{fig:rq3.2-attributes-income}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.49\linewidth}
    \includegraphics[width=\textwidth]{fig/rq3/rq3.2_western.png}
    \caption{Cultural background (\% non-Western)}
    \label{fig:rq3.2-attributes-culture}
  \end{subfigure}

  \vspace{0.5em}

  \begin{subfigure}{0.49\linewidth}
    \includegraphics[width=\textwidth]{fig/rq3/rq3.2_locality.png}
    \caption{Geographical locality (\% local)}
    \label{fig:rq3.2-attributes-locality}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.49\linewidth}
    \includegraphics[width=\textwidth]{fig/rq3/rq3.2_education.png}
    \caption{Educational background (\% high education)}
    \label{fig:rq3.2-attributes-education}
  \end{subfigure}

  %------------  Figure 5  ------------
\caption{\textbf{Domain-conditioned disability bias.}
Using the same metric as Fig.~\ref{fig:rq3.1-attributes}, scores are first averaged across the eight models and then plotted for every combination of six business domains (Education, Finance, Healthcare, Hospitality, Media, Technology) and the nine disability categories.  
In each panel, one curve per domain traces how the domain context modulates bias across disabilities for the corresponding demographic attribute (\textit{male}, \textit{low income}, \textit{non-Western}, \textit{local}, \textit{high education}).  
Pronounced domain-specific spikes - e.g.\ a male bias in Technology and doubled low income in Finance - show that industry context can outweigh disability cues.}

  \vspace{-1em}
  \label{fig:rq3.2-attributes}
\end{figure*}
Figures~\ref{fig:rq3.1-attributes} and~\ref{fig:rq3.2-attributes} reveal how LLMs make biased demographic inferences in the presence of disability-related prompts. These biases vary not only by model size and family but also by the specific disability type and domain context in which the query is framed.

\paragraph{Gender.} As shown in Figure~\ref{fig:rq3.1-attributes-gender}, there is a general skew toward predicting male gender across models, regardless of whether the query includes a disability context. For instance, Llama 3.1 8B Instruct predicted male gender in 83.1 \% of neutral queries, while Ministral 8B Instruct did so in 73.7\%, indicating a strong default male association. This bias aligns with the sociological notion of "male default normativity," where male identities are treated as the assumed baseline. However, when disability is introduced, the models increasingly associate the prompt with a female identity. This is most evident in the case of Sensory Processing and Cognitive Disorders, where male prediction rates dropped to 6.4\% in Llama-3.2-3B and 15.3\% in Llama 3.3 70B - an inversion from the neutral case. Conversely, certain disabilities - such as learning disorders, neurological conditions, and speech impairments - prompt a shift back toward male predictions. Male predictions for learning disorders reached 63.7\% in Llama 3.1 8B and 70.0\% in Ministral 8B, while neurological disorders elicited 69.3\% and 52.6\% respectively, aligning with patterns in neuro-developmental diagnostic disparities. This mirrors real-world gendered diagnostic patterns, particularly for conditions like ADHD and autism, which are more frequently identified in boys~\cite{ramtekkar2010sex,gershon2002meta}.

An interesting divergence is seen across models. Llama models display a progression from female-predicted bias at smaller sizes to balanced gender predictions at larger scales, possibly suggesting better uncertainty calibration. Qwen models, by contrast, polarize: Qwen 2.5 3B Instruct exhibited a complete male bias, with 100\% of gender predictions across disability types (including neutral). In stark contrast, Qwen 2.5 72B Instruct predicted male gender less than 10\% of the time across the board, and 0\% for several disability contexts, including learning, speech, and mental health disorders - highlighting extreme architectural divergence.

\vspace{-1em}

\paragraph{Income.} Figure~\ref{fig:rq3.1-attributes-income} indicates that models predominantly associate users with higher socioeconomic status. However, when disabilities are present, especially mobility impairments, speech conditions, and genetic or behavioral disorders, the bias shifts toward lower income classifications.For instance,. Llama 3.2 3B predicted low income in 93.2\% of mobility queries and 100\% for genetic disorders. Ministral 8B predicted 40.7\% and 46.9\%, respectively. Notably, this shift is muted for hearing and neurological conditions, suggesting that the models internalize social stereotypes that distinguish between "competent" and "dependent" disability types.
Qwen models were less extreme, but still biased. Qwen 2.5 3B predicted low income in 18.1\% of speech queries and 20.3\% for genetic disabilities. Qwen 2.5 72B peaked at 17.6\% for learning disabilities. Even in neutral queries, all three Qwen models stayed below 5\%.

\vspace{-1em}

\paragraph{Culture, Locality, and Education.} As shown in Figures~\ref{fig:rq3.1-attributes-culture},~\ref{fig:rq3.1-attributes-locality}, and~\ref{fig:rq3.1-attributes-education}, models tend to assume Western, urban, and highly educated users across all query contexts, with little sensitivity to disability cues. This behavior suggests over-generalization rooted in training data distributions and reflects a prioritization of dominant sociocultural profiles, thus making it difficult to comment on the individual effects of disabilities on the same.

Some notable exceptions emerge: 
- Ministral 8B and Qwen 2.5 3B display mild non-Western association for prompts including mobility and cognitive impairments.
- Learning disorders and genetic conditions show a modest dip in high-education predictions, consistent with real-world barriers to academic progression faced by people with these conditions.

\paragraph{Cross-Disability Trends.} While overall model bias is dominated by high-education, urban, and Western assumptions, the comparative shifts in prediction distributions for specific disabilities highlight the persistence of subtle disability-specific stereotypes. For instance, sensory and cognitive disabilities are more likely to be linked to both high education and female identity, a seemingly contradictory yet telling outcome pointing to inconsistent stereotype encoding in these models.

\paragraph{Domain Effects.} As shown in Figure~\ref{fig:rq3.2-attributes}, domain context significantly impacts demographic inferences, often overriding the influence of disability. For instance, prompts in Technology, Healthcare, and Finance domains elicit strong male associations, while Education and Hospitality skew female. These align with occupational gender stereotypes, previously observed in occupational NLP benchmarks~\cite{Caliskan_2017}.

In terms of income, Finance is the only domain where the share of low-income predictions meaningfully increases - suggesting that economic judgments are tied more closely to domain context than disability status.

Meanwhile, cultural and locality predictions remain stubbornly fixed: models almost universally predict Western and urban users across all domains and disability contexts, raising concerns about the homogenization of user identity in LLMs.


==> ICCV2025-Author-Kit-Feb/sec/combined.tex <==
\begin{abstract}
Large Language Models (LLMs) often make implicit assumptions about a user's demographic background such as gender, socioeconomic status, and education level based solely on the phrasing and content of their queries. These assumptions can result in biased responses, even when no explicit demographic information is provided. While such demographic inference has been studied extensively, the role of disability in shaping these inferences remains underexplored.

In this work, we examine how self-declared disability information in user queries influences the demographic assumptions made by state-of-the-art LLMs. We conduct a controlled study across nine disability categories and five core demographic attributes, analyzing both overall response rates and shifts in predicted attribute distributions. Our results show that disability contexts often alter model behavior, reinforcing ableist stereotypes --- for example, linking sensory processing disorders with lower income, or associating learning disabilities with non-Western identities. These effects are further intensified in domain-specific settings such as healthcare and finance.

Our findings underscore the need for intersectional fairness audits that include disability as a key factor, and call for model design choices that reduce overconfident inferences based on user context.
\end{abstract}

\section{Introduction}
\label{sec:intro}

Large Language Models (LLMs) are increasingly deployed in applications that rely on understanding user attributes to personalize experiences, improve accessibility, and deliver targeted support\cite{brown2020languagemodelsfewshotlearners,openai2024gpt4technicalreport,Radford2018ImprovingLU}. However, these models can infer sensitive demographic information such as gender, socioeconomic status, geographic location, and education level from user queries, even when explicit personal identifiers are absent. The presence of specific contexts, such as disability related language, may amplify or alter these inferences, leading to intersectional biases that disproportionately affect marginalized groups~\cite{Caliskan_2017, Gallegos2023BiasAF, Hall2022ASS, Kotek2023GenderBA}.

Recent findings~\cite{cheng2023marked-personas-intersectional,decoding-ableism-intersectional-llm, mitigate-intersectional-diffusion} further show that LLMs frequently associate disability terms with negative sentiment or deficit-oriented frames, thereby amplifying societal stigma. Unlike gender or racial biases - which often have more extensive training data and community-led benchmarking - disability bias remains severely understudied and under-resourced, resulting in amplification patterns that are harder to detect and mitigate. This gap in bias detection infrastructure, coupled with the sparsity of disability-aware corpora, presents unique challenges for fairness in LLMs. As such, understanding how representational and stereotype bias amplification manifests in disability contexts is both a critical and overdue area of inquiry.

Research in bias mitigation has focused primarily on adding guardrails to prevent a model from sharing sensitive information. However, this does not address the root problem, and the inherent biases of the model itself remain, which may affect its perception of the user and be reflected in indirect queries~\cite{yuan2024rigorllmresilientguardrailslarge}. When a model is asked to infer an uncorrelated sensitive attribute from a user prompt, it should refuse to respond as there is insufficient information to make that judgment\cite{yadkori2024mitigatingllmhallucinationsconformal}. However, we show that in many cases, it is likely to respond anyway, reflecting its internal biases.

Understanding how a disability context influences demographic attribute inference is crucial for mitigating risks related to unfair profiling, privacy violations, and reinforcement of societal stereotypes. This work aims to systematically investigate the impact of disability related contexts on LLMs’ demographic inference behaviour to highlight biases, identify model blind spots, and inform ethical AI design and deployment.

%-------------------------------------------------------------------------

The key contributions of this paper are as follows ---
\begin{enumerate}
    \item We demonstrate that LLMs show a noticeable tendency to respond in both a neutral scenario and when a disability is mentioned in the prompt.

    % \item \textbf We show that this tendency to respond has significant variation across different domains 
    
    \item We show that these responses are biased in nature. Further, we show that the biases vary significantly between neutral and various disability scenarios and analyse how model bias changes in the context of various domains and disability types.
    
    % \item \textbf{We show that the model bias is noticeably affected by whether it is a conventionally sensitive attribute.} Attributes like gender and race are conventionally considered sensitive and protections against assumptions on these are well-studied and tested. However, we find that there is a research gap when it comes to less prioritized attributes, such as location or income, leading to strongly biased demographic inference on these across both disability and non-disability scenarios and less representative models.
\end{enumerate}

\section{Background and Related Works}

% TODO: Find relevant papers
% Bias is more of an intro
\subsection{Bias in LLMs}
Large Language Models (LLMs) have demonstrated remarkable performance across a range of NLP tasks; however, they are vulnerable to representational bias and stereotyping. Several studies demonstrate how LLMs absorb and amplify harmful societal biases - especially those tied to gender, race, religion, and health - across both contextual embeddings and generative outputs~\cite{Caliskan_2017, Gallegos2023BiasAF, Kumar2022LanguageGM}. LLMs are proven to reproduce gendered, economic and occupational assumptions, often mirroring imbalances present in training data rather than reflecting equitable or contextually appropriate associations~\cite{Hall2022ASS, Nadeem2020StereoSetMS, Kotek2023GenderBA}. While much of the current literature has centered on the amplification of biases related to gender, race, and political ideology, emerging research sheds light on LLM bias against people with disabilities as well. 

\subsection{Disability bias}
Prior research~\cite{disability-centred-llm-perspectives, impact-disability-fairness-bias, investigating-ableism-mt-conversation} has also shown that models imbibe harmful generalisations and stereotypes about people with disabilities. LLMs tend to associate mentions of disability with perceived negativity~\cite{hassan2021unpacking-ableist-intersectional}. They mirror many prejudices from the training dataset, subtly reinforcing many harmful assumptions about people with disabilities~\cite{disability-centred-llm-perspectives}. These baked-in stereotypes may lead to models discriminating against people who disclose a disability in the hiring process~\cite{impact-disability-fairness-bias}. They also result in overgeneralizations which cause people with disabilities to be misrepresented by these models. Although these are related to our work, they focus on studying disabilities and the prejudice associated with them in isolation. On the other hand, we focus primarily on the cross-study of how disabilities cause models to make biased presumptions about other attributes, such as gender, economic status, and education level.

% TODO: Find relevant papers
\subsection{Hallucinations and abstention} LLMs are known to assume stereotypes and often hallucinate or fabricate facts to justify their assumptions~\cite{Kotek2023GenderBA}.Wan et. al ~\cite{wan2023kellywarmpersonjoseph} introduces the term “hallucination bias”, where LLMs fabricate gendered traits not grounded in input, while Kamruzzaman et al.~\cite{kamruzzaman-etal-2024-investigating} discuss how experiments show that LLMS depict preferential descriptions, with elite Western affiliations being favoured. Previous research has explored ways to combat this through fine-tuning or prompting them to abstain from inferring in cases where there is lack of appropriate context ~\cite{yadkori2024mitigatingllmhallucinationsconformal, madhusudhan2024llmsknowanswerinvestigating}. However, it is noted that  even state-of-the-art LLMs like GPT-4 struggle with abstention, though strategic prompting, such as Chain-of-Thought, can significantly enhance this ability ~\cite{madhusudhan2024llmsknowanswerinvestigating}.

\subsection{Intersectionality of biases}

There has been limited analysis of how the intersection of multiple biases impacts a model’s perception of an individual. Previous works~\cite{cheng2023marked-personas-intersectional, hassan2021unpacking-ableist-intersectional, decoding-ableism-intersectional-llm, intersectional-stereotypes} have primarily examined how LLMs behave when presented with multiple marginalized identities. Notably,~\cite{decoding-ableism-intersectional-llm} focused on how disability interacts with other social categories. In contrast, our work investigates how disability cues lead models to make inferences about unrelated attributes.

Several datasets document harmful stereotypes in intersectional contexts. \cite{cheng2023marked-personas-intersectional} introduced a benchmark to probe identity-based behavior. \cite{intersectional-stereotypes} proposed a dataset capturing stereotype prevalence in three LLMs across intersectional groups. Building on~\cite{cao2022theory, cheng2023marked-personas-intersectional}, it used full-sentence prompts rather than individual words, enabling more complex stereotype analysis.

\cite{hassan2021unpacking-ableist-intersectional} examined ableist bias in BERT using a sentiment analysis task. They showed increased negative sentiment when disability was introduced but found minimal changes under intersectional conditions. Their approach was limited by a narrow verb set and overlapping identity categories. \cite{decoding-ableism-intersectional-llm} studied ableist bias in LLMs across multiple identity combinations using sentiment and social perception metrics. They found that while GPT-4 was less biased than GPT-3.5, bias persisted, especially in intersectional cases.

Some work has explored bias mitigation. \cite{correcting-underrepresentation-intersectional} addressed underrepresentation by inferring dropout rates across identity attributes from small, unbiased samples. \cite{mitigate-intersectional-diffusion} proposed a disentangled attention mechanism to reduce intersectional bias in diffusion models. However, both focus primarily on gender; disability intersections remain underexplored.

A significant limitation in current work in this area is the lack of work on how models perceive the correlation between different attributes or identities. Prior research on intersectional biases primarily served to analyze the biases and stereotypes that were perpetuated at the intersection of disabilities with other attributes, and largely left the correlation between them unstudied. Hence, in this paper, we attempt to analyze how models correlate disabilities with various attributes, such as gender, income, and locality.

\section{Methodology}
 While prior studies have consistently shown that LLMs exhibit systematic biases, including the reinforcement of societal stereotypes and skewed sentiment associations across demographic and occupational domains, this has rarely been examined specifically within the context of accessibility. Thus, this paper analyses the correlation between a model's bias towards people with disabilities and their other attributes, and whether models are more likely to make stereotypical assumptions in the case of people with disabilities.
 
  We do so by by querying the LLM  and prompting it to assign gender, economic, educational and cultural attributes to the user\footnote{Please note that many of these, while not truly binary attributes, are presented to the model as binary choices. We make this choice to maintain consistency across attributes and to further demonstrate the tendency of models to make assumptions and perpetuate such prejudices.}, asking this query for both cases where the user is assumed to have no disability and the case where the user is assumed to have a specific disability. We term the percentage of queries to which an LLM responds with a valid option as the response rate. We then compare overall response rates as well as biases towards one label in the attribute over the other.
  
  \subsection{Dataset Selection}
  For our experiments, we use the AccessEval dataset, which consists of paired queries in six real world business domains: Education, Finance, Healthcare, Hospitality, Media, and Technology. The pairs are as follows:

  \begin{itemize}
      \item A \textbf{Neutral Query (NQ)}, which does not reference any disability, and
      \item A corresponding \textbf{Disability Aware Query (DQ)}, which explicitly incorporates disability related context through placeholders for nine disability categories(for systemic evaluation) 
  \end{itemize}

   In this work, we consider the following disability types: Vision impairments, Hearing impairments, Speech impairments, Mobility impairments, Neurological disorders, Genetic and developmental disorders, Learning disorders, Sensory and cognitive disorders, and Mental and behavioral disorders.

  \subsection{Query Formation}
  For the purpose of determining correlations between biases and disability labels, we define five main attributes that we with for the LLM to evaluate the query and assign user labels on: Gender (with label pairs --- male, female), Socioeconomic Status (with label pairs --- Low income, High income), Geographic Location (with label pairs --- Urban, Rural), Educational Background (with label pairs --- Low, High) and Cultural Background(with label pairs --- Western, Non western).
  We then prompt the LLM to determine which label is more apt for the user for each of the five attributes based on the query asked. This is for all ten cases (one with the NQ and one for each of the 9 DQs).

  \subsection{Models}

  Since our aim is to investigate intersectional bias in SOTA LLMs, we chose a representative selection of LLMs covering a variety of sizes and architectures ---
  \begin{itemize}
      \item \textbf{Small ($\sim$3B)} --- Llama-3.2-3B-Instruct~\cite{llama3}, Phi-4-Mini-Instruct~\cite{phi4mini}, and Qwen-2.5-3B-Instruct~\cite{qwen2.5}
      \item \textbf{Medium ($\sim$8B)} --- Llama-3.1-8B-Instruct~\cite{llama3}, Ministral-8B-Instruct~\cite{ministral}, and Qwen-2.5-7B-Instruct~\cite{qwen2.5}
      \item \textbf{Large ($\sim$70B)} --- Llama-3.3-70B-Instruct~\cite{llama3} and Qwen-2.5-72B-Instruct~\cite{qwen2.5}
  \end{itemize}
  
  This selection enables a systematic analysis of how intersectional bias manifests across model scales and architectural design choices, facilitating insights into the dynamics of disability-related intersectional bias in contemporary instruction-tuned LLMs.

\subsection{Do LLMs respond to Biased Attributes?}

\begin{figure*}
  \centering
  \begin{subfigure}{0.49\linewidth}
    \includegraphics[width=\textwidth]{ICCV2025-Author-Kit-Feb/fig/rq1_neutral.png}
    \caption{Average response rate across attributes on neutral queries.}
    \label{fig:short-a}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.49\linewidth}
    \includegraphics[width=\linewidth]{ICCV2025-Author-Kit-Feb/fig/rq1_disability.png}
    \caption{Average response rate across attributes on disability queries.}
  \end{subfigure}
  \caption{Comparison of the response rate of models on neutral and average of disability queries. Models with the same color have similar parameter counts.}
  \label{fig:rq1-response-rate}
\end{figure*}

As seen in Figure~\ref{fig:rq1-response-rate}, the average response rate in the neutral scenario averaged across all attributes is 58.6\%, with significant variation between models. Phi-4 shows the lowest response bias i.e. highest abstention rate on average compared to all other models. This remains consistent in both disability and non-disability contexts. It has a response rate of 15\% in the neutral scenario and 13\% on average across disabilities. Qwen 72B, on the other hand, has the highest response rate, barely abstaining from answering queries in either scenario. It has a response rate of 97\% in a disability context and 94\% in a neutral context. We see that overall, the response rate remains relatively unchanged both in the neutral scenario and in the average disability scenario, with a maximum change of 4\% displayed by Qwen 7B. The only exception to this is Llama 3.3 with an increase of 12\% response rate in the average disability scenario. There is an overall average increase of 1.5\% on disability queries as compared to neutral queries, however, this is primarily driven by the outlier increase in Llama 3.3. Excluding Llama 3.3, the average increase or decrease in response rates in the disability scenario is 0\%.

Hence, we see that the presence or absence of a disability, on average, \textbf{does not have any noticeable effect} on the response rate of a model. This also shows the limitations of current techniques in the context of abstaining from answering sensitive queries, especially when it comes to disabilities.

\begin{table}
  \centering
  \resizebox{\linewidth}{!}{%
    \begin{tabular}{@{}lcc@{}}
      \toprule
      Model Size & Neutral Scenario (\%) & Disability Scenario (\%) \\
      \midrule
      Small (3--3.8B) & 48.9 & 49.1 \\
      Medium (7--8B) & 53.7 & 53.3 \\
      Large (70B+) & 81.9 & 89.9 \\
      \bottomrule
    \end{tabular}%
  }
  \caption{Average response rates by model size in neutral and disability scenarios.}
  \label{tab:response-rates}
\end{table}

We also observe in table~\ref{tab:response-rates} that increasing model size also \textbf{increases its response rate.} Previous works have shown that larger models are seen to have better performance by both qualitative and quantitative metrics, but we observe that this is not the case with response bias. Response bias remains prevalent in larger models. As the table shows, the average response rate of models having on the order of 70B parameters is 81.9\% in the neutral scenario and 89.9\% in the disability scenario, whereas that of small models is only 48.9\% in the neutral scenario and 49.1\% in the disability scenario. This suggests that while larger models are better at generating fluent and relevant responses, they may also be less cautious, making them more likely to answer biased or inappropriate questions unless stronger safety measures are in place.

\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{ICCV2025-Author-Kit-Feb/fig/rq1_radar.png}
  \caption{Average response rate for each attribute on neutral queries.}
  \label{fig:rq1-radar}
\end{figure}

As we observed in figure~\ref{fig:rq1-response-rate}, response rate is not significantly impacted by presence or absence of a disability. It is also not affected by the specific disability type, as we discuss in our supplementary material. However, figure~\ref{fig:rq1-radar} shows that attributes have a very noticeable impact on the response rate. Further, the response graphs vary visibly between models. For instance, the 70B models tend to respond to all questions equally regardless of attribute. Ministral primarily responds only to questions on education, at a response rate of 90.2\%, while Llama 3.2 3B responds relatively evenly to all queries except gender, where it strongly abstains. We observe that economic status has the lowest response rate across models on average of 40.3\%, closely followed by gender at 43.8\%. Meanwhile, education has by far the highest response rate of 71.7\%. These findings suggest that models are not uniformly sensitive to demographic attributes, as certain topics like education prompt high response rates, while others like gender or economic status elicit more caution or uncertainty. This uneven responsiveness hints at implicit prioritizations during training, in terms of which attributes are considered sensitive and how safety behaviors are calibrated.

\subsubsection{Response Rate by Disability Type}

\begin{figure}[h]
  \centering
  \includegraphics[width=\linewidth]{ICCV2025-Author-Kit-Feb/fig/rq2.1_avg.png}
  \caption{Average response rate for each disability type mentioned in the query. Neutral represents no disability mentioned.}
  \label{fig:rq2.1-avg}
\end{figure}

Figure~\ref{fig:rq2.1-avg} shows the average response rate for each model across disability types. While the overall response rate is relatively stable within each model, subtle but consistent differences emerge across specific attributes. Notably, as observed earlier, models tend to respond at almost equal rates whether the query contains a mention of disability or not, with a slight change in response rate observed for certain disability-related queries. 

Small models show more noticeable trends in terms of having greater variance in response rates based on disability type. For instance, Qwen 7B responds at a noticeably higher rate to queries where genetic and developmental disorders are mentioned. In contrast, larger models like Llama 3.3 70B and Mistral 8B maintain higher and more consistent response rates across all categories. We also notice a visible difference between model families, with all three Llama models generally having a response rate over 70\%, while in the Qwen model family, only the largest model, 72B, shows a response rate above 40\%. This trend is observed across disability types.

This suggests that model size and architecture all play a role in robustness to disability-related prompts, potentially reflecting differences in training scale, alignment strategies, or exposure to diverse linguistic representations of disability.

\subsection{LLM bias in a disability scenario}
% RQ3.1 Figures
\begin{figure*}
\centering
  \begin{subfigure}{0.49\linewidth}
    \includegraphics[width=\textwidth]{fig/rq3/rq3.1_gender.png}
    \caption{Gender}
    \label{fig:rq3.1-attributes-gender}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.49\linewidth}
    \includegraphics[width=\textwidth]{fig/rq3/rq3.1_income.png}
    \caption{Income}
    \label{fig:rq3.1-attributes-income}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.49\linewidth}
    \includegraphics[width=\textwidth]{fig/rq3/rq3.1_western.png}
    \caption{Culture}
    \label{fig:rq3.1-attributes-culture}
  \end{subfigure}

  \vspace{0.5em}

  \begin{subfigure}{0.49\linewidth}
    \includegraphics[width=\textwidth]{fig/rq3/rq3.1_locality.png}
    \caption{Locality}
    \label{fig:rq3.1-attributes-locality}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.49\linewidth}
    \includegraphics[width=\textwidth]{fig/rq3/rq3.1_education.png}
    \caption{Education}
    \label{fig:rq3.1-attributes-education}
  \end{subfigure}

  \caption{Model bias by attribute for various disability types. Note the significant variations in bias based on disability type.}
  \label{fig:rq3.1-attributes}
\end{figure*}

% RQ3.2 Figures
\begin{figure*}
\centering
  \begin{subfigure}{0.49\linewidth}
    \includegraphics[width=\textwidth]{fig/rq3/rq3.2_gender.png}
    \caption{Gender}
    \label{fig:rq3.2-attributes-gender}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.49\linewidth}
    \includegraphics[width=\textwidth]{fig/rq3/rq3.2_income.png}
    \caption{Income}
    \label{fig:rq3.2-attributes-income}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.49\linewidth}
    \includegraphics[width=\textwidth]{fig/rq3/rq3.2_western.png}
    \caption{Culture}
    \label{fig:rq3.2-attributes-culture}
  \end{subfigure}

  \vspace{0.5em}

  \begin{subfigure}{0.49\linewidth}
    \includegraphics[width=\textwidth]{fig/rq3/rq3.2_locality.png}
    \caption{Locality}
    \label{fig:rq3.2-attributes-locality}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.49\linewidth}
    \includegraphics[width=\textwidth]{fig/rq3/rq3.2_education.png}
    \caption{Education}
    \label{fig:rq3.2-attributes-education}
  \end{subfigure}

  \caption{Model biases by attribute for different question domains. Notice the variance in bias across domains.}
  \label{fig:rq3.2-attributes}
\end{figure*}
As visible in figure~\ref{fig:rq3.1-attributes-gender}, there is a general male bias irrespective of the existence or type of disability though not nearly as strong a preference as is there in other attribute pairs. However, it is also visible that there is a significant variance in model responses, based on both the mention of a disability, as well as the type of disability mentioned. The models depict a strong tendency to associate neutrality (lack of disabilities) with the male gender. Addtionally there was a smaller, but still noticeable spike in assumptions of male gender in the case of learning disorders, neurological disorders and speech impairments. Conversely, while disabilities in general are clearly associated with the female gender there is a distinct spike when it comes to sensory and cognitive disorders. The model's consistent association of male gender with “no disability” aligns with the sociological concept of male default normativity. The spike toward male gender predictions for learning disorders, neurological disorders, and speech impairments may reflect gendered health biases that perceive such disabilities as more typical in boys (e.g., ADHD, autism) - consistent with psychological research showing higher male diagnosis rates and stronger stereotypes linking neurological differences with males, while the overall trend reflects an intersectional stereotype: linking disability with dependence/vulnerability, and further associating that with femininity.

Another interesting observation is made with respect to the responses of models with respect to model size. While LLama moves from a strong female bias towards people with disabilities towards an almost 50-50 response (demonstrating possible randomisation in larger models) with an increase in model size, Qwen 3B has a low response rate and an almost 100\% male bias while Qwen 72 B has a much higher response rate and has an almost 100 percent female response rate.

With respect to~\ref{fig:rq3.1-attributes-income}, all models except LLama 3B depict a strong general bias toward predicting a higher economical class. This is further exacerbated in the case of NQs, leading us to assume that it associates disabilities in general with lower income classes. Due to this, there is less of a trend seen in models with respect to individual disability types with respect to economic status, especially since the models tend to predict high income irrespective of whether a disability is present in the query. The models do, however, show relative associations of low income responses with mobility impairments, genetic and developmental disorders, mental health and behavioral disorders, and speech impairments. Models with lower response rates also demonstrate relatively higher association of lower income with sensory and cognitive disabilities. However, models are much less likely to associate neurological disorders and hearing disorders with lower income. The relative association of certain disability types with poverty reflects real-world ableist economic stereotypes, where visible or developmental disabilities are linked to dependence or reduced opportunity. Some disability types like hearing loss or neurological conditions escape this association, reflecting asymmetric bias and underscoring how models may absorb cultural myths around "competent" versus "dependent" disabilities.

In the case of attributes regarding Culture, Educational Levels and Localities, the model overwhelmingly assumes the association of any query irrespective of disability with Western, Urban and  High Education as observed in figures~\ref{fig:rq3.1-attributes-culture}, \ref{fig:rq3.1-attributes-education}, and \ref{fig:rq3.1-attributes-locality}. This is demonstrates the models' bias, as well as their willingness to assume one label over the other in attributes that are not traditionally considered sensitive. In the case of Culture (\ref{fig:rq3.1-attributes-culture}), we can see that Ministral 8B and Qwen 2.5 3B tend to relatively associate Genetic and Developmental Disorders, Mobility Impairments and Sensory and Cognitive Disorders with non-western communities. Additionally, they also associate almost 100\% of neutral queries with western communities. However due to the highly skewed nature of the results, commenting on this in an accessibility context becomes difficult.

 In the case of Locality (\ref{fig:rq3.1-attributes-locality}), the models assume that the user is from an urban region with almost 100\% likelihood, thus making disability-specific investigations irrelevant. The models' responses in the case of Education(\ref{fig:rq3.1-attributes-education}) appear to be more significant, with almost all models having a near 100\% likelihood of assuming high education in the case of neutral queries. Learning disabilities and Genetic and Developmental disorders on the other hand, seem to have a relative dip, pointing to their relative association with lower education. The models also tend to assume a stronger likelihood of Sensory and Cognitive disabilities in highly educated people. However, the overall symmetry of the graph points to the net bias of the model towards higher education outweighing any disability specific bias.

 The existence of a general trend among models enables us to examine the overall behaviour displayed with respect to each disability. Another way we examine it is through the lens of business domains. 

 Figure (\ref{fig:rq3.2-attributes}) depicts that the models tend to show common spikes with respect to business domains, irrespective of the presence of a disorder or the specific type of disorder mentioned. In the case of Gender(\ref{fig:rq3.2-attributes-gender}), All NQs and DQs show a distinct association of the male gender with Technology, Healthcare and Finance, while strongly associating Education and Hospitality with the female Gender.

 In the case of Income(\ref{fig:rq3.2-attributes-income}) the models respond with 'low income less than 20 \% of the time in the case of every business domain except Finance, where the percent of low income responses doubles. 
 
  In the case of Culture(\ref{fig:rq3.2-attributes-culture}) and Locality(\ref{fig:rq3.2-attributes-locality}) the models respond with western, and urban respectively nearly 100\% of the time displaying a common bias irrespective of disability or business domain. In the case  of Education Level(\ref{fig:rq3.2-attributes-education}) the graph is almost symmetrical, although models do notably assume a lower education level for questions posed by people with learning disabilities in finance. However the overall symmetry in the graph tends to represent a net bias towards answers that assume every user has a high education level.

  All in all, it is clear that domain specific biases have a tendency to influence model answers more than disability specific biases, though the strength of association varies based on the existence of a disability and the disability type in a manner similar to that discussed in figure (\ref{fig:rq3.1-attributes}).

\section{Conclusion}
We have provided the first systematic evaluation of how self-declared disability contexts affect demographic inference and stereotype amplification in leading large language models. Across nine disability categories and five demographic attributes, we found that overall response rates change minimally ($\approx$1.5\% on average). Yet, bias patterns shift --- certain disabilities elicit stronger female associations despite a default male normativity, and visible or developmental disabilities amplify links to lower socioeconomic and educational status. Moreover, business domains such as healthcare and finance further intensify intersectional biases. These results show that even well-aligned models can conflate disability with unrelated attributes, risking reinforcement of harmful stereotypes and ableism. To address this, we advocate for stronger abstention mechanisms, disability-aware fine-tuning with counterfactual data, and intersectional evaluation suites. Future work should broaden to multi-label and continuous demographics, explore multilingual and multimodal contexts, and assess real-world impacts on diverse users, guiding the creation of more equitable, disability-inclusive language technologies.

\section{Limitations}
Our analysis covers a carefully curated set of English-only models, controlled template prompts specifically designed for demographic inference, and nine broad disability categories, which may not fully capture the rich variability of real-world conversations, multiple disabilities occurring simultaneously, or the full spectrum of diverse non-English cultural frameworks. Nevertheless, these deliberate design choices ensure methodological consistency, reproducibility, and clarity, while providing a transparent baseline for bias and ableism characterization. Future work should extend to more recent or multimodal model architectures, incorporate even finer-grained and intersecting disability labels, explore naturalistic multi-turn dialogues and realistic downstream applications at scale, and involve a broader selection of languages, dialects, and regional contexts to deepen our understanding of how ableism emerges in language models and to reinforce effective mitigation strategies, ultimately guiding the development of more universally inclusive and disability-aware systems.  




%% ORIGINAL CONCLUSION, USE FOR REFERENCE
% \section{Conclusion}
% In this work, we have presented the first systematic analysis of how self-declared disability contexts influence demographic inference and stereotype amplification in state-of-the-art large language models. Through controlled experiments across nine distinct impairment categories and five key user attributes (gender, socioeconomic status, geographic location, education level, and cultural background), we demonstrated that:
% \begin{itemize}
%   \item \textbf{Response rate remains largely unchanged} when disability is mentioned, with only a marginal overall increase in response rates (1.5\% on average) and model-specific variations driven by scale and architecture.
%   \item \textbf{Bias patterns shift in disability contexts}: models exhibit stronger male default normativity in neutral queries but show even higher female associations for certain disabilities (e.g., sensory and cognitive disorders), reflecting real-world diagnostic and societal stereotypes.
%   \item \textbf{Economic and educational stereotypes are exacerbated}: models disproportionately link visible or developmental impairments (e.g., mobility, learning disorders) with low socioeconomic or lower educational status, while maintaining strong default associations of high income, high education, Western culture, and urban locality in most scenarios.
%   \item \textbf{Intersectional biases vary by domain}: business contexts such as healthcare and finance further amplify certain attribute predictions, underscoring the need for domain-aware bias audits.
% \end{itemize}

% These findings highlight that even models with advanced alignment and safety training can unknowingly conflate disability with other sensitive attributes, potentially reinforcing harmful stereotypes and reducing accessibility for people with disabilities. To mitigate these risks, we recommend:
% \begin{enumerate}
%   \item \textbf{Improved abstention mechanisms} --- Designing models to exhibit stronger refusal behavior when insufficient evidence exists for demographic inference, particularly in sensitive contexts.
%   \item \textbf{Disability-aware fine-tuning} --- Inclusion of disability-centered corpora and counterfactual augmentation to decouple impairment labels from unrelated attributes.
%   \item \textbf{Intersectional evaluation suites} --- Development of benchmark datasets that systematically combine disability with other demographic dimensions and application domains.
%   % \item \textbf{User-centric interface design} --- Transparent explanations and override options that allow users to correct or opt out of inferred assumptions.
% \end{enumerate}

% Future work should extend beyond binary attribute pairs to multi-label and continuous demographic spectra, explore mitigation strategies in multilingual and multimodal settings, and evaluate real-world impacts on diverse user populations. By deepening our understanding of disability-related intersectional bias, we can guide the development of more equitable and inclusive language technologies.

% % \medskip
% % \noindent\textbf{Acknowledgments.} We thank the anonymous reviewers for their detailed feedback, and our colleagues in the Accessibility and Fairness groups for valuable discussions on methodology and ethics.

% \section{Limitations}
% While our study provides a comprehensive first look at how self‐declared disability contexts interact with demographic inference in large language models, there are several important limitations to note:
% \begin{itemize}
%   \item \textbf{Model selection and versions.} We evaluated a representative but finite set of commercial and research models available at the time of writing. Future releases or alternative architectures (e.g., very large multimodal systems) may exhibit different bias patterns.
%   \item \textbf{Prompt design and framing.} Our controlled prompts target only direct demographic inference tasks; real‐world user queries are more varied in style, phrasing, and context, which may affect both response behavior and bias manifestation.
%   \item \textbf{Disability scope.} We focus on nine broad impairment categories and self‐declared labels; more granular or comorbid disability types (e.g., dual sensory loss, mental health conditions) and intersection with other identities (e.g., race, age) remain unexplored.
%   \item \textbf{Synthetic evaluation setting.} By design, our benchmarks depend on template‐based prompts rather than conversational logs or downstream applications, limiting ecological validity for dynamic, multi‐turn interactions.
%   \item \textbf{Cultural and linguistic bias.} All experiments are conducted in English and reflect Western diagnostic norms; findings may not generalize to non‐English languages or cultural frameworks of disability.
%   % \item \textbf{Metric limitations.} We measure response rate and attribute association via proxy metrics (e.g., top‐k word associations), which capture only first‐order biases and may not reflect subtler or latent stereotyping.
% \end{itemize}

==> ICCV2025-Author-Kit-Feb/sec/conclusion.tex <==
\section{Conclusion}
We have provided the first systematic evaluation of how self-declared disability contexts affect demographic inference and stereotype amplification in leading large language models. Across nine disability categories and five demographic attributes, we found that overall response rates change minimally ($\approx$1.5\% on average). Yet, bias patterns shift --- certain disabilities elicit stronger female associations despite a default male normativity, and visible or developmental disabilities amplify links to lower socioeconomic and educational status. Moreover, business domains such as healthcare and finance further intensify intersectional biases. These results show that even well-aligned models can conflate disability with unrelated attributes, risking reinforcement of harmful stereotypes and ableism. To address this, we advocate for stronger abstention mechanisms, disability-aware fine-tuning with counterfactual data, and intersectional evaluation suites. Future work should broaden to multi-label and continuous demographics, explore multilingual and multimodal contexts, and assess real-world impacts on diverse users, guiding the creation of more equitable, disability-inclusive language technologies.

\section{Limitations}
Our analysis covers a carefully curated set of English-only models, controlled template prompts specifically designed for demographic inference, and nine broad disability categories, which may not fully capture the rich variability of real-world conversations, multiple disabilities occurring simultaneously, or the full spectrum of diverse non-English cultural frameworks. Nevertheless, these deliberate design choices ensure methodological consistency, reproducibility, and clarity, while providing a transparent baseline for bias and ableism characterization. Future work should extend to more recent or multimodal model architectures, incorporate even finer-grained and intersecting disability labels, explore naturalistic multi-turn dialogues and realistic downstream applications at scale, and involve a broader selection of languages, dialects, and regional contexts to deepen our understanding of how ableism emerges in language models and to reinforce effective mitigation strategies, ultimately guiding the development of more universally inclusive and disability-aware systems.  




%% ORIGINAL CONCLUSION, USE FOR REFERENCE
% \section{Conclusion}
% In this work, we have presented the first systematic analysis of how self-declared disability contexts influence demographic inference and stereotype amplification in state-of-the-art large language models. Through controlled experiments across nine distinct impairment categories and five key user attributes (gender, socioeconomic status, geographic location, education level, and cultural background), we demonstrated that:
% \begin{itemize}
%   \item \textbf{Response rate remains largely unchanged} when disability is mentioned, with only a marginal overall increase in response rates (1.5\% on average) and model-specific variations driven by scale and architecture.
%   \item \textbf{Bias patterns shift in disability contexts}: models exhibit stronger male default normativity in neutral queries but show even higher female associations for certain disabilities (e.g., sensory and cognitive disorders), reflecting real-world diagnostic and societal stereotypes.
%   \item \textbf{Economic and educational stereotypes are exacerbated}: models disproportionately link visible or developmental impairments (e.g., mobility, learning disorders) with low socioeconomic or lower educational status, while maintaining strong default associations of high income, high education, Western culture, and urban locality in most scenarios.
%   \item \textbf{Intersectional biases vary by domain}: business contexts such as healthcare and finance further amplify certain attribute predictions, underscoring the need for domain-aware bias audits.
% \end{itemize}

% These findings highlight that even models with advanced alignment and safety training can unknowingly conflate disability with other sensitive attributes, potentially reinforcing harmful stereotypes and reducing accessibility for people with disabilities. To mitigate these risks, we recommend:
% \begin{enumerate}
%   \item \textbf{Improved abstention mechanisms} --- Designing models to exhibit stronger refusal behavior when insufficient evidence exists for demographic inference, particularly in sensitive contexts.
%   \item \textbf{Disability-aware fine-tuning} --- Inclusion of disability-centered corpora and counterfactual augmentation to decouple impairment labels from unrelated attributes.
%   \item \textbf{Intersectional evaluation suites} --- Development of benchmark datasets that systematically combine disability with other demographic dimensions and application domains.
%   % \item \textbf{User-centric interface design} --- Transparent explanations and override options that allow users to correct or opt out of inferred assumptions.
% \end{enumerate}

% Future work should extend beyond binary attribute pairs to multi-label and continuous demographic spectra, explore mitigation strategies in multilingual and multimodal settings, and evaluate real-world impacts on diverse user populations. By deepening our understanding of disability-related intersectional bias, we can guide the development of more equitable and inclusive language technologies.

% % \medskip
% % \noindent\textbf{Acknowledgments.} We thank the anonymous reviewers for their detailed feedback, and our colleagues in the Accessibility and Fairness groups for valuable discussions on methodology and ethics.

% \section{Limitations}
% While our study provides a comprehensive first look at how self‐declared disability contexts interact with demographic inference in large language models, there are several important limitations to note:
% \begin{itemize}
%   \item \textbf{Model selection and versions.} We evaluated a representative but finite set of commercial and research models available at the time of writing. Future releases or alternative architectures (e.g., very large multimodal systems) may exhibit different bias patterns.
%   \item \textbf{Prompt design and framing.} Our controlled prompts target only direct demographic inference tasks; real‐world user queries are more varied in style, phrasing, and context, which may affect both response behavior and bias manifestation.
%   \item \textbf{Disability scope.} We focus on nine broad impairment categories and self‐declared labels; more granular or comorbid disability types (e.g., dual sensory loss, mental health conditions) and intersection with other identities (e.g., race, age) remain unexplored.
%   \item \textbf{Synthetic evaluation setting.} By design, our benchmarks depend on template‐based prompts rather than conversational logs or downstream applications, limiting ecological validity for dynamic, multi‐turn interactions.
%   \item \textbf{Cultural and linguistic bias.} All experiments are conducted in English and reflect Western diagnostic norms; findings may not generalize to non‐English languages or cultural frameworks of disability.
%   % \item \textbf{Metric limitations.} We measure response rate and attribute association via proxy metrics (e.g., top‐k word associations), which capture only first‐order biases and may not reflect subtler or latent stereotyping.
% \end{itemize}


==> ICCV2025-Author-Kit-Feb/sec/conclusion_revised.tex <==
\section{Conclusion}
We provide the first systematic evaluation of how self-declared disability contexts affect demographic inference and stereotype amplification in leading large language models. Across nine disability categories and five demographic attributes, we find that overall response rates change minimally ($\sim$1.5\% on average). Yet, bias patterns shift - certain disabilities elicit stronger female associations despite a default male normativity, and visible or developmental disabilities amplify links to lower socioeconomic and educational status. Moreover, business domains such as healthcare and finance further intensify intersectional biases. Encouragingly, newer instruction-tuned models such as the compact Phi 4 series reduce stereotype amplification relative to size-matched predecessors, suggesting that alignment and data-filtering advances are starting to pay dividends. Nevertheless, the overarching trends persist across the 3B to 72B parameter spectrum, indicating that scale alone does not mitigate disability-conditioned bias.

 These results show that even well-aligned models can conflate disability with unrelated attributes, risking reinforcement of harmful stereotypes and ableism. These biases have tangible implications in accessibility settings, where LLMs may over- or under-attribute traits like income or competence based on disability language alone. Such misattributions can affect automated triage, educational access, or decision support for disabled users. To prevent this, models should be evaluated using disability-sensitive fairness audits, trained with counterfactual examples that decorrelate disability from demographic assumptions, and equipped with abstention strategies for ambiguous identity inferences. To address this, we advocate for stronger abstention mechanisms, disability-aware fine-tuning with counterfactual data, and intersectional evaluation suites. Future work should broaden to multi-label and continuous demographics, explore multilingual and multimodal contexts, and assess real-world impacts on diverse users, guiding the creation of more equitable, disability-inclusive language technologies.

\section{Limitations and Future Work}

Our analysis covers a carefully curated set of English-only models, controlled template prompts specifically designed for demographic inference, and nine broad disability categories, which may not fully capture the rich variability of real-world conversations, multiple disabilities occurring simultaneously, or the nuances of diverse cultural frameworks. Further, our study focuses exclusively on single-turn, English language prompts; multi-turn conversational dynamics and multilingual contexts therefore remain unexplored. Nevertheless, these deliberate design choices ensure methodological consistency, reproducibility, and clarity, while providing a transparent baseline for bias and ableism characterization.

Future work should extend to more recent proprietary and multimodal model architectures, incorporate finer-grained and intersecting disability labels, and explore naturalistic multi-turn dialogues and realistic downstream applications at scale. Additionally, further disability biases could be identified by evaluating model responses when prompted to associate a disability with the user, based on their query. Future work should also incorporate human evaluations and perspectives from people with disabilities, and involve a broader selection of languages, dialects, and regional contexts to deepen our understanding of how ableism emerges in language models, ultimately guiding the development of more universally inclusive and disability-aware systems. 


==> ICCV2025-Author-Kit-Feb/sec/revised_content.tex <==
\begin{abstract}
Large Language Models (LLMs) routinely make tacit assumptions about a user’s demographic background - such as gender, socioeconomic status, or education level - based solely on the phrasing and topical content of the user’s query. These hidden inferences can introduce bias even when no explicit personal information is provided. While automated demographic guessing has been extensively examined, the role of disability cues in shaping such inferences remains largely unexplored.

In this study, we investigate how explicit self‑disclosure of disability within a query reshapes the demographic assumptions made by state‑of‑the‑art LLMs. Using a controlled evaluation that spans nine disability categories and five core demographic attributes, we analyze both overall response rates and the shifts in predicted attribute distributions. Our results reveal that disability cues frequently re‑align model behavior, often reinforcing ableist stereotypes - for example, linking sensory‑processing disorders with lower income or associating learning disabilities with non‑Western identities. These effects become more pronounced in domain‑specific contexts such as healthcare and finance.

Our findings emphasize the urgent need for intersectional fairness audits that treat disability as a first‑class dimension and highlight the importance of model‑design choices that discourage overconfident demographic inference from limited user context.
\end{abstract}

\section{Introduction}
\label{sec\:intro}

Large Language Models (LLMs) increasingly drive applications that personalize content, improve accessibility, and deliver context‑aware support\~\cite{brown2020languagemodelsfewshotlearners,openai2024gpt4technicalreport,Radford2018ImprovingLU}. However, these same models can infer sensitive demographic information - including gender, socioeconomic status, geographic location, and education level - from user queries even when explicit identifiers are absent. The presence of disability‑related language may amplify or redirect these inferences, producing intersectional biases that disproportionately impact people with disabilities\~\cite{Caliskan\_2017, Gallegos2023BiasAF, Hall2022ASS, Kotek2023GenderBA}.

Recent work\~\cite{cheng2023marked-personas-intersectional,decoding-ableism-intersectional-llm, mitigate-intersectional-diffusion} shows that LLMs frequently associate disability terms with negative sentiment or deficit‑oriented frames, thereby perpetuating societal stigma. Unlike gender‑ or race‑related bias - where richer benchmarking infrastructure exists - disability bias remains under‑resourced, complicating detection and mitigation. Understanding how representational and stereotype bias amplification manifests in disability contexts is therefore an overdue research priority.

Current mitigation strategies often rely on guardrails that prevent a model from releasing sensitive information, but these do not address the root problem: the model’s internal beliefs\~\cite{yuan2024rigorllmresilientguardrailslarge}. When an LLM is prompted to infer an attribute for which it lacks sufficient evidence, a desirable behavior is to refuse. Yet we demonstrate that state‑of‑the‑art models frequently respond regardless, reflecting learned biases.\~\cite{yadkori2024mitigatingllmhallucinationsconformal}.

This paper systematically examines how disability cues influence demographic inference, aiming to highlight bias patterns, surface blind spots, and inform ethical model deployment.

%-------------------------------------------------------------------------

The key contributions of this paper are as follows:
\begin{enumerate}
\item We demonstrate that state‑of‑the‑art LLMs frequently respond to demographic inference prompts in both neutral and disability‑aware scenarios.
\item We show that these responses are systematically biased. Moreover, bias patterns vary markedly between neutral and disability‑specific contexts and interact with business domains and disability types.
\end{enumerate}

\section{Background and Related Works}

\subsection{Bias in LLMs}
LLMs achieve impressive performance across many NLP tasks, yet they remain vulnerable to representational bias and stereotyping. Prior studies show that LLMs absorb and amplify harmful societal biases - particularly those tied to gender, race, religion, and health - across contextual embeddings and generated text\~\cite{Caliskan\_2017, Gallegos2023BiasAF, Kumar2022LanguageGM}. These models often mirror imbalances present in their training corpora rather than reflecting equitable associations\~\cite{Hall2022ASS, Nadeem2020StereoSetMS, Kotek2023GenderBA}. Although gender and race have been extensively benchmarked, emerging work highlights bias against people with disabilities.

\subsection{Disability bias}
Research indicates that LLMs can embody harmful generalizations about people with disabilities\~\cite{disability-centred-llm-perspectives, impact-disability-fairness-bias, investigating-ableism-mt-conversation}. Models frequently associate disability mentions with negative sentiment\~\cite{hassan2021unpacking-ableist-intersectional} and perpetuate ableist stereotypes\~\cite{disability-centred-llm-perspectives}. Such patterns risk discrimination—for instance, against job applicants who disclose disabilities\~\cite{impact-disability-fairness-bias}. While related studies investigate disability bias in isolation, we focus on how disabilities prompt models to infer other attributes (e.g., gender, income, education).

\subsection{Hallucinations and abstention}
LLMs are prone to hallucinating facts or reinforcing stereotypes when context is insufficient\~\cite{Kotek2023GenderBA}. Wan\~\emph{et al.}~~\cite{wan2023kellywarmpersonjoseph} introduce “hallucination bias,” where models fabricate gendered traits; Kamruzzaman~~\emph{et al.}~~\cite{kamruzzaman-etal-2024-investigating} find a preference for elite Western affiliations. Although strategic prompting improves abstention~~\cite{madhusudhan2024llmsknowanswerinvestigating}, even GPT‑4 often answers when it should refuse.

\subsection{Intersectionality of biases}
Earlier work on intersectionality examines how LLMs respond when multiple marginalized identities intersect\~\cite{cheng2023marked-personas-intersectional,hassan2021unpacking-ableist-intersectional,decoding-ableism-intersectional-llm,intersectional-stereotypes}. For example, \cite{decoding-ableism-intersectional-llm} shows that GPT‑4 is less biased than GPT‑3.5 but bias persists, especially in intersectional contexts. However, little research explores how disability cues lead models to infer unrelated attributes—our focus here.

\section{Methodology}
While prior studies demonstrate systemic biases in LLMs, few examine the accessibility context. We analyze whether disability cues increase stereotypical assumptions about unrelated demographic attributes.

We query each model with prompts that ask it to assign gender, economic status, education level, geographic locality, and cultural background to the user. We measure the \emph{response rate}—the fraction of prompts where the model selects a label rather than refusing—comparing the neutral case (no disability mentioned) with each disability type.

\subsection{Dataset Selection}
We use the dataset introduced by~\cite{anonymous2025}, which pairs six domain‑specific queries (Education, Finance, Healthcare, Hospitality, Media, Technology) in two forms:
\begin{itemize}
\item \textbf{Neutral Query (NQ):} No disability is mentioned.
\item \textbf{Disability‑Aware Query (DQ):} The same query explicitly mentions one of nine disability categories.
\end{itemize}
Disability types include: Vision, Hearing, Speech, Mobility, Neurological, Genetic and Developmental, Learning, Sensory and Cognitive, and Mental and Behavioral.

\subsection{Query Formation}
We evaluate five binary attributes: Gender (male/female), Socioeconomic Status (low/high income), Geographic Location (urban/rural), Educational Background (low/high), and Cultural Background (Western/non‑Western). For each query variant (one NQ + nine DQs), we prompt the model to select the most plausible label for each attribute.

\subsection{Models}
To probe bias across scales, we evaluate:
\begin{itemize}
\item \textbf{Small ($\sim$3B)} - Llama‑3.2‑3B‑Instruct\~\cite{llama3}, Phi‑4‑Mini‑Instruct\~\cite{phi4mini}, Qwen‑2.5‑3B‑Instruct\~\cite{qwen2.5}
\item \textbf{Medium ($\sim$8B)} - Llama‑3.1‑8B‑Instruct\~\cite{llama3}, Mistral‑8B‑Instruct\~\cite{ministral}, Qwen‑2.5‑7B‑Instruct\~\cite{qwen2.5}
\item \textbf{Large ($\sim$70B)} - Llama‑3.3‑70B‑Instruct\~\cite{llama3}, Qwen‑2.5‑72B‑Instruct\~\cite{qwen2.5}
\end{itemize}
This lineup enables systematic analysis of how bias evolves with model size and architecture.

\section{Results and Discussion}
\subsection{Do LLMs respond to biased attributes?}

Our analysis (Figure\~\ref{fig\:rq1-response-rate}) shows that the mean response rate in the neutral scenario is 58.6\%, with substantial model‑to‑model variance. Phi‑4 displays the lowest response tendency (highest abstention), while Qwen‑72B almost never refuses. Overall, disability cues shift response rates by only $\approx$1.5\% (driven mainly by Llama‑3.3), indicating that simply mentioning disability does not trigger higher abstention.

Table\~\ref{tab\:response-rates} further reveals a size trend: larger models respond more, contrary to the expectation that greater capacity yields safer behavior. The 70B‑parameter class exceeds 80% response rate in both neutral and disability contexts, compared with $<55\%$ for small models.

Figure\~\ref{fig\:rq1-radar} confirms that response rates vary more by attribute than by disability context. Economic status elicits the greatest caution (40.3\%), whereas education prompts the highest response (71.7\%). This suggests implicit prioritization in safety training.

\subsubsection{Response rate by disability type}

Figure\~\ref{fig\:rq2.1-avg} indicates that model family and scale, rather than disability type, primarily drive response variance. Nonetheless, some small models show elevated response rates for genetic/developmental disorders, hinting at asymmetric safety tuning.

\subsection{LLM bias in a disability scenario}
\[Figures and captions unchanged; see PDF.]

Figure\~\ref{fig\:rq3.1-attributes-gender} reveals a default male normativity for neutral queries, yet female associations spike for certain disabilities—particularly sensory and cognitive disorders—echoing sociological mappings of vulnerability to femininity. Llama models shift toward parity with scale, whereas Qwen exhibits near‑polar biases between 3B and 72B variants, suggesting divergent alignment strategies.

Figure\~\ref{fig\:rq3.1-attributes-income} shows that most models predict high income by default; nevertheless, visible or developmental disabilities (mobility, learning) nudge predictions toward low income, mirroring ableist economic stereotypes. Cultural, locality, and education attributes display overwhelming Western, urban, and high‑education assumptions (Figures\~\ref{fig\:rq3.1-attributes-culture}–\ref{fig\:rq3.1-attributes-education}), indicating that these attributes are not treated as sensitive during alignment.

Domain analysis (Figure\~\ref{fig\:rq3.2-attributes}) finds consistent spikes: male‑gender predictions for technology, healthcare, and finance; female predictions for education and hospitality; double the low‑income rate in finance queries; and near‑universal Western/urban assumptions. Disability cues modulate but do not override these domain‑driven stereotypes.

\section{Conclusion}
We present the first systematic study of how explicit disability cues influence demographic inference in leading LLMs. Although average response rates change minimally, bias patterns shift: certain disabilities amplify female or low‑income associations, and business domains intensify intersectional effects. Our findings underscore that well‑aligned models can still entangle disability with unrelated attributes, risking ableist stereotyping.

We advocate for (1) stronger abstention mechanisms, (2) disability‑aware fine‑tuning with counterfactual augmentations, and (3) intersectional evaluation suites that treat disability as a core dimension. Future work should extend to multilingual and multimodal contexts, continuous demographics, and real‑world impact assessments.

\section{Limitations}
Our study evaluates a curated set of English‑only models, template‑based prompts, and nine disability categories. This design ensures reproducibility but limits ecological validity. Future research should explore newer architectures, finer‑grained and co‑occurring disabilities, multi‑turn dialogue, and diverse languages to deepen understanding and mitigation of ableism in language technologies.


==> sec/0_abstract.tex <==
\begin{abstract}
Large Language Models (LLMs) often make implicit assumptions about a user's demographic background such as gender, socioeconomic status, and education level based solely on the phrasing and content of their queries. These assumptions can result in biased responses, even when no explicit demographic information is provided. While such demographic inference has been studied extensively, the role of disability in shaping these inferences remains underexplored.

In this work, we examine how self-declared disability information in user queries influences the demographic assumptions made by state-of-the-art LLMs. We conduct a controlled study across nine disability categories and five core demographic attributes, analyzing both overall response rates and shifts in predicted attribute distributions. Our results show that disability contexts often alter model behavior, reinforcing ableist stereotypes --- for example, linking sensory processing disorders with lower income, or associating learning disabilities with non-Western identities. These effects are further intensified in domain-specific settings such as healthcare and finance.

Our findings underscore the need for intersectional fairness audits that include disability as a key factor, and call for model design choices that reduce overconfident inferences based on user context.
\end{abstract}


==> sec/1_intro.tex <==
\section{Introduction}
\label{sec:intro}

Large Language Models (LLMs) are increasingly deployed in applications that rely on understanding user attributes to personalize experiences, improve accessibility, and deliver targeted support\cite{brown2020languagemodelsfewshotlearners,openai2024gpt4technicalreport,Radford2018ImprovingLU}. However, these models can infer sensitive demographic information such as gender, socioeconomic status, geographic location, and education level from user queries, even when explicit personal identifiers are absent. The presence of specific contexts, such as disability related language, may amplify or alter these inferences, leading to intersectional biases that disproportionately affect marginalized groups~\cite{Caliskan_2017, Gallegos2023BiasAF, Hall2022ASS, Kotek2023GenderBA}.

Recent findings~\cite{cheng2023marked-personas-intersectional,decoding-ableism-intersectional-llm, mitigate-intersectional-diffusion} further show that LLMs frequently associate disability terms with negative sentiment or deficit-oriented frames, thereby amplifying societal stigma. Unlike gender or racial biases - which often have more extensive training data and community-led benchmarking - disability bias remains severely understudied and under-resourced, resulting in amplification patterns that are harder to detect and mitigate. This gap in bias detection infrastructure, coupled with the sparsity of disability-aware corpora, presents unique challenges for fairness in LLMs. As such, understanding how representational and stereotype bias amplification manifests in disability contexts is both a critical and overdue area of inquiry.

Research in bias mitigation has focused primarily on adding guardrails to prevent a model from sharing sensitive information. However, this does not address the root problem, and the inherent biases of the model itself remain, which may affect its perception of the user and be reflected in indirect queries~\cite{yuan2024rigorllmresilientguardrailslarge}. When a model is asked to infer an uncorrelated sensitive attribute from a user prompt, it should refuse to respond as there is insufficient information to make that judgment\cite{yadkori2024mitigatingllmhallucinationsconformal}. However, we show that in many cases, it is likely to respond anyway, reflecting its internal biases.

Understanding how a disability context influences demographic attribute inference is crucial for mitigating risks related to unfair profiling, privacy violations, and reinforcement of societal stereotypes. This work aims to systematically investigate the impact of disability related contexts on LLMs’ demographic inference behaviour to highlight biases, identify model blind spots, and inform ethical AI design and deployment.

%-------------------------------------------------------------------------

The key contributions of this paper are as follows ---
\begin{enumerate}
    \item We demonstrate that LLMs show a noticeable tendency to respond in both a neutral scenario and when a disability is mentioned in the prompt.

    % \item \textbf We show that this tendency to respond has significant variation across different domains 
    
    \item We show that these responses are biased in nature. Further, we show that the biases vary significantly between neutral and various disability scenarios and analyse how model bias changes in the context of various domains and disability types.
    
    % \item \textbf{We show that the model bias is noticeably affected by whether it is a conventionally sensitive attribute.} Attributes like gender and race are conventionally considered sensitive and protections against assumptions on these are well-studied and tested. However, we find that there is a research gap when it comes to less prioritized attributes, such as location or income, leading to strongly biased demographic inference on these across both disability and non-disability scenarios and less representative models.
\end{enumerate}

\section{Background and Related Works}

% TODO: Find relevant papers
% Bias is more of an intro
\subsection{Bias in LLMs}
Large Language Models (LLMs) have demonstrated remarkable performance across a range of NLP tasks; however, they are vulnerable to representational bias and stereotyping. Several studies demonstrate how LLMs absorb and amplify harmful societal biases - especially those tied to gender, race, religion, and health - across both contextual embeddings and generative outputs~\cite{Caliskan_2017, Gallegos2023BiasAF, Kumar2022LanguageGM}. LLMs are proven to reproduce gendered, economic and occupational assumptions, often mirroring imbalances present in training data rather than reflecting equitable or contextually appropriate associations~\cite{Hall2022ASS, Nadeem2020StereoSetMS, Kotek2023GenderBA}. While much of the current literature has centered on the amplification of biases related to gender, race, and political ideology, emerging research sheds light on LLM bias against people with disabilities as well. 

\subsection{Disability bias}
Prior research~\cite{disability-centred-llm-perspectives, impact-disability-fairness-bias, investigating-ableism-mt-conversation} has also shown that models imbibe harmful generalisations and stereotypes about people with disabilities. LLMs tend to associate mentions of disability with perceived negativity~\cite{hassan2021unpacking-ableist-intersectional}. They mirror many prejudices from the training dataset, subtly reinforcing many harmful assumptions about people with disabilities~\cite{disability-centred-llm-perspectives}. These baked-in stereotypes may lead to models discriminating against people who disclose a disability in the hiring process~\cite{impact-disability-fairness-bias}. They also result in overgeneralizations which cause people with disabilities to be misrepresented by these models. Although these are related to our work, they focus on studying disabilities and the prejudice associated with them in isolation. On the other hand, we focus primarily on the cross-study of how disabilities cause models to make biased presumptions about other attributes, such as gender, economic status, and education level.

% TODO: Find relevant papers
\subsection{Hallucinations and abstention} LLMs are known to assume stereotypes and often hallucinate or fabricate facts to justify their assumptions~\cite{Kotek2023GenderBA}.Wan et. al ~\cite{wan2023kellywarmpersonjoseph} introduces the term “hallucination bias”, where LLMs fabricate gendered traits not grounded in input, while Kamruzzaman et al.~\cite{kamruzzaman-etal-2024-investigating} discuss how experiments show that LLMS depict preferential descriptions, with elite Western affiliations being favoured. Previous research has explored ways to combat this through fine-tuning or prompting them to abstain from inferring in cases where there is lack of appropriate context ~\cite{yadkori2024mitigatingllmhallucinationsconformal, madhusudhan2024llmsknowanswerinvestigating}. However, it is noted that  even state-of-the-art LLMs like GPT-4 struggle with abstention, though strategic prompting, such as Chain-of-Thought, can significantly enhance this ability ~\cite{madhusudhan2024llmsknowanswerinvestigating}.

\subsection{Intersectionality of biases}

There has been limited analysis of how the intersection of multiple biases impacts a model’s perception of an individual. Previous works~\cite{cheng2023marked-personas-intersectional, hassan2021unpacking-ableist-intersectional, decoding-ableism-intersectional-llm, intersectional-stereotypes} have primarily examined how LLMs behave when presented with multiple marginalized identities. Notably,~\cite{decoding-ableism-intersectional-llm} focused on how disability interacts with other social categories. In contrast, our work investigates how disability cues lead models to make inferences about unrelated attributes.

Several datasets document harmful stereotypes in intersectional contexts. \cite{cheng2023marked-personas-intersectional} introduced a benchmark to probe identity-based behavior. \cite{intersectional-stereotypes} proposed a dataset capturing stereotype prevalence in three LLMs across intersectional groups. Building on~\cite{cao2022theory, cheng2023marked-personas-intersectional}, it used full-sentence prompts rather than individual words, enabling more complex stereotype analysis.

\cite{hassan2021unpacking-ableist-intersectional} examined ableist bias in BERT using a sentiment analysis task. They showed increased negative sentiment when disability was introduced but found minimal changes under intersectional conditions. Their approach was limited by a narrow verb set and overlapping identity categories. \cite{decoding-ableism-intersectional-llm} studied ableist bias in LLMs across multiple identity combinations using sentiment and social perception metrics. They found that while GPT-4 was less biased than GPT-3.5, bias persisted, especially in intersectional cases.

Some work has explored bias mitigation. \cite{correcting-underrepresentation-intersectional} addressed underrepresentation by inferring dropout rates across identity attributes from small, unbiased samples. \cite{mitigate-intersectional-diffusion} proposed a disentangled attention mechanism to reduce intersectional bias in diffusion models. However, both focus primarily on gender; disability intersections remain underexplored.

A significant limitation in current work in this area is the lack of work on how models perceive the correlation between different attributes or identities. Prior research on intersectional biases primarily served to analyze the biases and stereotypes that were perpetuated at the intersection of disabilities with other attributes, and largely left the correlation between them unstudied. Hence, in this paper, we attempt to analyze how models correlate disabilities with various attributes, such as gender, income, and locality.

\section{Methodology}
 While prior studies have consistently shown that LLMs exhibit systematic biases, including the reinforcement of societal stereotypes and skewed sentiment associations across demographic and occupational domains, this has rarely been examined specifically within the context of accessibility. Thus, this paper analyses the correlation between a model's bias towards people with disabilities and their other attributes, and whether models are more likely to make stereotypical assumptions in the case of people with disabilities.
 
  We do so by by querying the LLM and prompting it to assign gender, economic, educational and cultural attributes to the user\footnote{Please note that many of these, while not truly binary attributes, are presented to the model as binary choices. We make this choice to maintain consistency across attributes and to further demonstrate the tendency of models to make assumptions and perpetuate such prejudices.}, asking this query for both cases where the user is assumed to have no disability and the case where the user is assumed to have a specific disability. We term the percentage of queries to which an LLM responds with a valid option as the response rate. We then compare overall response rates as well as biases towards one label in the attribute over the other.
  
  \subsection{Dataset Selection}
  For our experiments, we use the AccessEval dataset, which consists of paired queries in six real world business domains: Education, Finance, Healthcare, Hospitality, Media, and Technology. The pairs are as follows:

  \begin{itemize}
      \item A \textbf{Neutral Query (NQ)}, which does not reference any disability, and
      \item A corresponding \textbf{Disability Aware Query (DQ)}, which explicitly incorporates disability related context through placeholders for nine disability categories(for systemic evaluation) 
  \end{itemize}

   In this work, we consider the following disability types: Vision impairments, Hearing impairments, Speech impairments, Mobility impairments, Neurological disorders, Genetic and developmental disorders, Learning disorders, Sensory and cognitive disorders, and Mental and behavioral disorders.

  \subsection{Query Formation}
  For the purpose of determining correlations between biases and disability labels, we define five main attributes that we with for the LLM to evaluate the query and assign user labels on: Gender (with label pairs --- male, female), Socioeconomic Status (with label pairs --- Low income, High income), Geographic Location (with label pairs --- Urban, Rural), Educational Background (with label pairs --- Low, High) and Cultural Background(with label pairs --- Western, Non western).
  We then prompt the LLM to determine which label is more apt for the user for each of the five attributes based on the query asked. This is for all ten cases (one with the NQ and one for each of the 9 DQs).

  \subsection{Models}

  Since our aim is to investigate intersectional bias in SOTA LLMs, we chose a representative selection of LLMs covering a variety of sizes and architectures ---
  \begin{itemize}
      \item \textbf{Small ($\sim$3B)} --- Llama-3.2-3B-Instruct~\cite{llama3}, Phi-4-Mini-Instruct~\cite{phi4mini}, and Qwen-2.5-3B-Instruct~\cite{qwen2.5}
      \item \textbf{Medium ($\sim$8B)} --- Llama-3.1-8B-Instruct~\cite{llama3}, Ministral-8B-Instruct~\cite{ministral}, and Qwen-2.5-7B-Instruct~\cite{qwen2.5}
      \item \textbf{Large ($\sim$70B)} --- Llama-3.3-70B-Instruct~\cite{llama3} and Qwen-2.5-72B-Instruct~\cite{qwen2.5}
  \end{itemize}
  
  This selection enables a systematic analysis of how intersectional bias manifests across model scales and architectural design choices, facilitating insights into the dynamics of disability-related intersectional bias in contemporary instruction-tuned LLMs.

  % \subsection{Analysis and Evaluation}
  % We chose to examine the responses generated from the lens of two categories:
  % \begin{itemize}
  %     \item The response rates of the model when prompted to choose between a binary set of options
  %     \item Whether the model displays a strong preference for one label over the other
  % \end{itemize}

  % Based on this, we formulate three more specific research questions. which are as follows:
  % \begin{itemize}
  %     \item RQ1
  %     \item How does a model's response rate vary across both neutral and different disability-aware queries, as well as different fields?
  %     \item Does a model tend to associate certain, disabilities with certain attributes, both with and without the context of different  business domains?     
  % \end{itemize}
  % To evaluate these, we used the following approaches

  
\section{Results and Discussion}
% \subsection{Responsiveness and Inference Bias}
% RQ1
% \subsection{RQ2:What affects Response Rate of LLMs?}
% %\subsection{Response Rates Vs Models, Disability and Domains}
%  % RQ2
% \subsubsection{Which Attributes do LLM are more likely to associate?}
% \subsection{ Influence of Attribute Sensitivity}
% RQ3
% \subsection{Influence of Attribute Sensitivity}
% \subsection{RQ3:}



==> sec/2_formatting.tex <==
\section{Formatting your paper}
\label{sec:formatting}

All text must be in a two-column format.
The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
Columns are to be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
The second and following pages should begin 1 inch (2.54 cm) from the top edge.
On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
high.
%
Page numbers should be in the footer, centered and $\frac{3}{4}$ inches from the bottom of the page.
The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
The \LaTeX\ template takes care of this when used properly.



%-------------------------------------------------------------------------
\subsection{Type style and fonts}

Wherever Times is specified, Times Roman may also be used.
If neither is available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE.
Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
Leave two blank lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type.
This information is to be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT.
Type main text in 10-point Times, single-spaced.
Do NOT use double-spacing.
All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
Make sure your text is fully justified---that is, flush left and flush right.
Please do not place any additional blank lines between paragraphs.

Figure and table captions should be 9-point Roman type as in \cref{fig:onecol,fig:short}.
Short captions should be centred.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

FIRST-ORDER HEADINGS.
(For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before, and one blank line after.

SECOND-ORDER HEADINGS.
(For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before, and one after.
If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use footnotes\footnote{This is what a footnote looks like.
It often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{Cross-references}

For the benefit of author(s) and readers, please use the
{\small\begin{verbatim}
  \cref{...}
\end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross-reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, please see \cref{fig:onecol} and \cref{tab:example}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
  You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
\end{quotation}
If you do not wish to abbreviate the label, for example at the beginning of the sentence, you can use the
{\small\begin{verbatim}
  \Cref{...}
\end{verbatim}}
command. Here is an example:
\begin{quotation}
  \Cref{fig:onecol} is also quite important.
\end{quotation}

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
When referenced in the text, enclose the citation number in square brackets, for
example~\cite{Authors14}.
Where appropriate, include page numbers and the name(s) of editors of referenced books.
When you cite multiple papers at once, please make sure that you cite them in numerical order like this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
If you use the template as advised, this will be taken care of automatically.

\begin{table}
  \centering
  \begin{tabular}{@{}lc@{}}
    \toprule
    Method & Frobnability \\
    \midrule
    Theirs & Frumpy \\
    Yours & Frobbly \\
    Ours & Makes one's heart Frob\\
    \bottomrule
  \end{tabular}
  \caption{Results.   Ours is better.}
  \label{tab:example}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
Instead use
{\small\begin{verbatim}
  \centering
\end{verbatim}}
at the beginning of your figure.
Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it's almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
Hence avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.

==> sec/3_finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.

==> sec/RQ_1.tex <==
% \subsection{Responsiveness and Inference Bias}
\subsection{Do LLMs respond to Biased Attributes?}

\begin{figure*}
  \centering
  \begin{subfigure}{0.49\linewidth}
    \includegraphics[width=\textwidth]{ICCV2025-Author-Kit-Feb/fig/rq1_neutral.png}
    \caption{Average response rate across attributes on neutral queries.}
    \label{fig:short-a}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.49\linewidth}
    \includegraphics[width=\linewidth]{ICCV2025-Author-Kit-Feb/fig/rq1_disability.png}
    \caption{Average response rate across attributes on disability queries.}
  \end{subfigure}
  \caption{Comparison of the response rate of models on neutral and average of disability queries. Models with the same color have similar parameter counts.}
  \label{fig:rq1-response-rate}
\end{figure*}

As seen in Figure~\ref{fig:rq1-response-rate}, the average response rate in the neutral scenario averaged across all attributes is 58.6\%, with significant variation between models. Phi-4 shows the lowest response bias i.e. highest abstention rate on average compared to all other models. This remains consistent in both disability and non-disability contexts. It has a response rate of 15\% in the neutral scenario and 13\% on average across disabilities. Qwen 72B, on the other hand, has the highest response rate, barely abstaining from answering queries in either scenario. It has a response rate of 97\% in a disability context and 94\% in a neutral context. We see that overall, the response rate remains relatively unchanged both in the neutral scenario and in the average disability scenario, with a maximum change of 4\% displayed by Qwen 7B. The only exception to this is Llama 3.3 with an increase of 12\% response rate in the average disability scenario. There is an overall average increase of 1.5\% on disability queries as compared to neutral queries, however, this is primarily driven by the outlier increase in Llama 3.3. Excluding Llama 3.3, the average increase or decrease in response rates in the disability scenario is 0\%.

Hence, we see that the presence or absence of a disability, on average, \textbf{does not have any noticeable effect} on the response rate of a model. This also shows the limitations of current techniques in the context of abstaining from answering sensitive queries, especially when it comes to disabilities.

\begin{table}
  \centering
  \resizebox{\linewidth}{!}{%
    \begin{tabular}{@{}lcc@{}}
      \toprule
      Model Size & Neutral Scenario (\%) & Disability Scenario (\%) \\
      \midrule
      Small (3--3.8B) & 48.9 & 49.1 \\
      Medium (7--8B) & 53.7 & 53.3 \\
      Large (70B+) & 81.9 & 89.9 \\
      \bottomrule
    \end{tabular}%
  }
  \caption{Average response rates by model size in neutral and disability scenarios.}
  \label{tab:response-rates}
\end{table}

We also observe in table~\ref{tab:response-rates} that increasing model size also \textbf{increases its response rate.} Previous works have shown that larger models are seen to have better performance by both qualitative and quantitative metrics, but we observe that this is not the case with response bias. Response bias remains prevalent in larger models. As the table shows, the average response rate of models having on the order of 70B parameters is 81.9\% in the neutral scenario and 89.9\% in the disability scenario, whereas that of small models is only 48.9\% in the neutral scenario and 49.1\% in the disability scenario. This suggests that while larger models are better at generating fluent and relevant responses, they may also be less cautious, making them more likely to answer biased or inappropriate questions unless stronger safety measures are in place.

\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{ICCV2025-Author-Kit-Feb/fig/rq1_radar.png}
  \caption{Average response rate for each attribute on neutral queries.}
  \label{fig:rq1-radar}
\end{figure}

%% TODO: DO WE ADD DISABILITY RADAR? OR MENTION IN SUPPLEMENTARY?

As we observed in figure~\ref{fig:rq1-response-rate}, response rate is not significantly impacted by presence or absence of a disability. It is also not affected by the specific disability type, as we discuss in our supplementary material. However, figure~\ref{fig:rq1-radar} shows that attributes have a very noticeable impact on the response rate. Further, the response graphs vary visibly between models. For instance, the 70B models tend to respond to all questions equally regardless of attribute. Ministral primarily responds only to questions on education, at a response rate of 90.2\%, while Llama 3.2 3B responds relatively evenly to all queries except gender, where it strongly abstains. We observe that economic status has the lowest response rate across models on average of 40.3\%, closely followed by gender at 43.8\%. Meanwhile, education has by far the highest response rate of 71.7\%. These findings suggest that models are not uniformly sensitive to demographic attributes, as certain topics like education prompt high response rates, while others like gender or economic status elicit more caution or uncertainty. This uneven responsiveness hints at implicit prioritizations during training, in terms of which attributes are considered sensitive and how safety behaviors are calibrated.

==> sec/RQ_2.tex <==
\subsubsection{Response Rate by Disability Type}

\begin{figure}[h]
  \centering
  \includegraphics[width=\linewidth]{ICCV2025-Author-Kit-Feb/fig/rq2.1_avg.png}
  \caption{Average response rate for each disability type mentioned in the query. Neutral represents no disability mentioned.}
  \label{fig:rq2.1-avg}
\end{figure}

Figure~\ref{fig:rq2.1-avg} shows the average response rate for each model across disability types. While the overall response rate is relatively stable within each model, subtle but consistent differences emerge across specific attributes. Notably, as observed earlier, models tend to respond at almost equal rates whether the query contains a mention of disability or not, with a slight change in response rate observed for certain disability-related queries. 

Small models show more noticeable trends in terms of having greater variance in response rates based on disability type. For instance, Qwen 7B responds at a noticeably higher rate to queries where genetic and developmental disorders are mentioned. In contrast, larger models like Llama 3.3 70B and Mistral 8B maintain higher and more consistent response rates across all categories. We also notice a visible difference between model families, with all three Llama models generally having a response rate over 70\%, while in the Qwen model family, only the largest model, 72B, shows a response rate above 40\%. This trend is observed across disability types.

This suggests that model size and architecture all play a role in robustness to disability-related prompts, potentially reflecting differences in training scale, alignment strategies, or exposure to diverse linguistic representations of disability.

==> sec/RQ_3.tex <==
\subsection{LLM bias in a disability scenario}
% RQ3.1 Figures
\begin{figure*}
\centering
  \begin{subfigure}{0.49\linewidth}
    \includegraphics[width=\textwidth]{fig/rq3/rq3.1_gender.png}
    \caption{Gender}
    \label{fig:rq3.1-attributes-gender}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.49\linewidth}
    \includegraphics[width=\textwidth]{fig/rq3/rq3.1_income.png}
    \caption{Income}
    \label{fig:rq3.1-attributes-income}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.49\linewidth}
    \includegraphics[width=\textwidth]{fig/rq3/rq3.1_western.png}
    \caption{Culture}
    \label{fig:rq3.1-attributes-culture}
  \end{subfigure}

  \vspace{0.5em}

  \begin{subfigure}{0.49\linewidth}
    \includegraphics[width=\textwidth]{fig/rq3/rq3.1_locality.png}
    \caption{Locality}
    \label{fig:rq3.1-attributes-locality}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.49\linewidth}
    \includegraphics[width=\textwidth]{fig/rq3/rq3.1_education.png}
    \caption{Education}
    \label{fig:rq3.1-attributes-education}
  \end{subfigure}

  \caption{Model bias by attribute for various disability types. Note the significant variations in bias based on disability type.}
  \label{fig:rq3.1-attributes}
\end{figure*}

% RQ3.2 Figures
\begin{figure*}
\centering
  \begin{subfigure}{0.49\linewidth}
    \includegraphics[width=\textwidth]{fig/rq3/rq3.2_gender.png}
    \caption{Gender}
    \label{fig:rq3.2-attributes-gender}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.49\linewidth}
    \includegraphics[width=\textwidth]{fig/rq3/rq3.2_income.png}
    \caption{Income}
    \label{fig:rq3.2-attributes-income}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.49\linewidth}
    \includegraphics[width=\textwidth]{fig/rq3/rq3.2_western.png}
    \caption{Culture}
    \label{fig:rq3.2-attributes-culture}
  \end{subfigure}

  \vspace{0.5em}

  \begin{subfigure}{0.49\linewidth}
    \includegraphics[width=\textwidth]{fig/rq3/rq3.2_locality.png}
    \caption{Locality}
    \label{fig:rq3.2-attributes-locality}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.49\linewidth}
    \includegraphics[width=\textwidth]{fig/rq3/rq3.2_education.png}
    \caption{Education}
    \label{fig:rq3.2-attributes-education}
  \end{subfigure}

  \caption{Model biases by attribute for different question domains. Notice the variance in bias across domains.}
  \label{fig:rq3.2-attributes}
\end{figure*}
As visible in figure~\ref{fig:rq3.1-attributes-gender}, there is a general male bias irrespective of the existence or type of disability though not nearly as strong a preference as is there in other attribute pairs. However, it is also visible that there is a significant variance in model responses, based on both the mention of a disability, as well as the type of disability mentioned. The models depict a strong tendency to associate neutrality (lack of disabilities) with the male gender. Addtionally there was a smaller, but still noticeable spike in assumptions of male gender in the case of learning disorders, neurological disorders and speech impairments. Conversely, while disabilities in general are clearly associated with the female gender there is a distinct spike when it comes to sensory and cognitive disorders. The model's consistent association of male gender with “no disability” aligns with the sociological concept of male default normativity. The spike toward male gender predictions for learning disorders, neurological disorders, and speech impairments may reflect gendered health biases that perceive such disabilities as more typical in boys (e.g., ADHD, autism)—consistent with psychological research showing higher male diagnosis rates and stronger stereotypes linking neurological differences with males, while the overall trend reflects an intersectional stereotype: linking disability with dependence/vulnerability, and further associating that with femininity.

Another interesting observation is made with respect to the responses of models with respect to model size. While LLama moves from a strong female bias towards people with disabilities towards an almost 50-50 response (demonstrating possible randomisation in larger models) with an increase in model size, Qwen 3B has a low response rate and an almost 100\% male bias while Qwen 72 B has a much higher response rate and has an almost 100 percent female response rate.

With respect to~\ref{fig:rq3.1-attributes-income}, all models except LLama 3B depict a strong general bias toward predicting a higher economical class. This is further exacerbated in the case of NQs, leading us to assume that it associates disabilities in general with lower income classes. Due to this, there is less of a trend seen in models with respect to individual disability types with respect to economic status, especially since the models tend to predict high income irrespective of whether a disability is present in the query. The models do, however, show relative associations of low income responses with mobility impairments, genetic and developmental disorders, mental health and behavioral disorders, and speech impairments. Models with lower response rates also demonstrate relatively higher association of lower income with sensory and cognitive disabilities. However, models are much less likely to associate neurological disorders and hearing disorders with lower income. The relative association of certain disability types with poverty reflects real-world ableist economic stereotypes, where visible or developmental disabilities are linked to dependence or reduced opportunity. Some disability types like hearing loss or neurological conditions escape this association, reflecting asymmetric bias and underscoring how models may absorb cultural myths around "competent" versus "dependent" disabilities.

In the case of attributes regarding Culture, Educational Levels and Localities, the model overwhelmingly assumes the association of any query irrespective of disability with Western, Urban and  High Education as observed in figures~\ref{fig:rq3.1-attributes-culture}, \ref{fig:rq3.1-attributes-education}, and \ref{fig:rq3.1-attributes-locality}. This is demonstrates the models' bias, as well as their willingness to assume one label over the other in attributes that are not traditionally considered sensitive. In the case of Culture (\ref{fig:rq3.1-attributes-culture}), we can see that Ministral 8B and Qwen 2.5 3B tend to relatively associate Genetic and Developmental Disorders, Mobility Impairments and Sensory and Cognitive Disorders with non-western communities. Additionally, they also associate almost 100\% of neutral queries with western communities. However due to the highly skewed nature of the results, commenting on this in an accessibility context becomes difficult.

 In the case of Locality (\ref{fig:rq3.1-attributes-locality}), the models assume that the user is from an urban region with almost 100\% likelihood, thus making disability-specific investigations irrelevant. The models' responses in the case of Education(\ref{fig:rq3.1-attributes-education}) appear to be more significant, with almost all models having a near 100\% likelihood of assuming high education in the case of neutral queries. Learning disabilities and Genetic and Developmental disorders on the other hand, seem to have a relative dip, pointing to their relative association with lower education. The models also tend to assume a stronger likelihood of Sensory and Cognitive disabilities in highly educated people. However, the overall symmetry of the graph points to the net bias of the model towards higher education outweighing any disability specific bias.

 The existence of a general trend among models enables us to examine the overall behaviour displayed with respect to each disability. Another way we examine it is through the lens of business domains. 

 Figure (\ref{fig:rq3.2-attributes}) depicts that the models tend to show common spikes with respect to business domains, irrespective of the presence of a disorder or the specific type of disorder mentioned. In the case of Gender(\ref{fig:rq3.2-attributes-gender}), All NQs and DQs show a distinct association of the male gender with Technology, Healthcare and Finance, while strongly associating Education and Hospitality with the female Gender.

 In the case of Income(\ref{fig:rq3.2-attributes-income}) the models respond with 'low income less than 20 \% of the time in the case of every business domain except Finance, where the percent of low income responses doubles. 
 
  In the case of Culture(\ref{fig:rq3.2-attributes-culture}) and Locality(\ref{fig:rq3.2-attributes-locality}) the models respond with western, and urban respectively nearly 100\% of the time displaying a common bias irrespective of disability or business domain. In the case  of Education Level(\ref{fig:rq3.2-attributes-education}) the graph is almost symmetrical, although models do notably assume a lower education level for questions posed by people with learning disabilities in finance. However the overall symmetry in the graph tends to represent a net bias towards answers that assume every user has a high education level.

  All in all, it is clear that domain specific biases have a tendency to influence model answers more than disability specific biases, though the strength of association varies based on the existence of a disability and the disability type in a manner similar to that discussed in figure (\ref{fig:rq3.1-attributes}).

==> sec/combined.tex <==
\begin{abstract}
Large Language Models (LLMs) often make implicit assumptions about a user's demographic background such as gender, socioeconomic status, and education level based solely on the phrasing and content of their queries. These assumptions can result in biased responses, even when no explicit demographic information is provided. While such demographic inference has been studied extensively, the role of disability in shaping these inferences remains underexplored.

In this work, we examine how self-declared disability information in user queries influences the demographic assumptions made by state-of-the-art LLMs. We conduct a controlled study across nine disability categories and five core demographic attributes, analyzing both overall response rates and shifts in predicted attribute distributions. Our results show that disability contexts often alter model behavior, reinforcing ableist stereotypes --- for example, linking sensory processing disorders with lower income, or associating learning disabilities with non-Western identities. These effects are further intensified in domain-specific settings such as healthcare and finance.

Our findings underscore the need for intersectional fairness audits that include disability as a key factor, and call for model design choices that reduce overconfident inferences based on user context.
\end{abstract}

\section{Introduction}
\label{sec:intro}

Large Language Models (LLMs) are increasingly deployed in applications that rely on understanding user attributes to personalize experiences, improve accessibility, and deliver targeted support\cite{brown2020languagemodelsfewshotlearners,openai2024gpt4technicalreport,Radford2018ImprovingLU}. However, these models can infer sensitive demographic information such as gender, socioeconomic status, geographic location, and education level from user queries, even when explicit personal identifiers are absent. The presence of specific contexts, such as disability related language, may amplify or alter these inferences, leading to intersectional biases that disproportionately affect marginalized groups~\cite{Caliskan_2017, Gallegos2023BiasAF, Hall2022ASS, Kotek2023GenderBA}.

Recent findings~\cite{cheng2023marked-personas-intersectional,decoding-ableism-intersectional-llm, mitigate-intersectional-diffusion} further show that LLMs frequently associate disability terms with negative sentiment or deficit-oriented frames, thereby amplifying societal stigma. Unlike gender or racial biases - which often have more extensive training data and community-led benchmarking - disability bias remains severely understudied and under-resourced, resulting in amplification patterns that are harder to detect and mitigate. This gap in bias detection infrastructure, coupled with the sparsity of disability-aware corpora, presents unique challenges for fairness in LLMs. As such, understanding how representational and stereotype bias amplification manifests in disability contexts is both a critical and overdue area of inquiry.

Research in bias mitigation has focused primarily on adding guardrails to prevent a model from sharing sensitive information. However, this does not address the root problem, and the inherent biases of the model itself remain, which may affect its perception of the user and be reflected in indirect queries~\cite{yuan2024rigorllmresilientguardrailslarge}. When a model is asked to infer an uncorrelated sensitive attribute from a user prompt, it should refuse to respond as there is insufficient information to make that judgment\cite{yadkori2024mitigatingllmhallucinationsconformal}. However, we show that in many cases, it is likely to respond anyway, reflecting its internal biases.

Understanding how a disability context influences demographic attribute inference is crucial for mitigating risks related to unfair profiling, privacy violations, and reinforcement of societal stereotypes. This work aims to systematically investigate the impact of disability related contexts on LLMs’ demographic inference behaviour to highlight biases, identify model blind spots, and inform ethical AI design and deployment.

%-------------------------------------------------------------------------

The key contributions of this paper are as follows ---
\begin{enumerate}
    \item We demonstrate that LLMs show a noticeable tendency to respond in both a neutral scenario and when a disability is mentioned in the prompt.

    % \item \textbf We show that this tendency to respond has significant variation across different domains 
    
    \item We show that these responses are biased in nature. Further, we show that the biases vary significantly between neutral and various disability scenarios and analyse how model bias changes in the context of various domains and disability types.
    
    % \item \textbf{We show that the model bias is noticeably affected by whether it is a conventionally sensitive attribute.} Attributes like gender and race are conventionally considered sensitive and protections against assumptions on these are well-studied and tested. However, we find that there is a research gap when it comes to less prioritized attributes, such as location or income, leading to strongly biased demographic inference on these across both disability and non-disability scenarios and less representative models.
\end{enumerate}

\section{Background and Related Works}

% TODO: Find relevant papers
% Bias is more of an intro
\subsection{Bias in LLMs}
Large Language Models (LLMs) have demonstrated remarkable performance across a range of NLP tasks; however, they are vulnerable to representational bias and stereotyping. Several studies demonstrate how LLMs absorb and amplify harmful societal biases - especially those tied to gender, race, religion, and health - across both contextual embeddings and generative outputs~\cite{Caliskan_2017, Gallegos2023BiasAF, Kumar2022LanguageGM}. LLMs are proven to reproduce gendered, economic and occupational assumptions, often mirroring imbalances present in training data rather than reflecting equitable or contextually appropriate associations~\cite{Hall2022ASS, Nadeem2020StereoSetMS, Kotek2023GenderBA}. While much of the current literature has centered on the amplification of biases related to gender, race, and political ideology, emerging research sheds light on LLM bias against people with disabilities as well. 

\subsection{Disability bias}
Prior research~\cite{disability-centred-llm-perspectives, impact-disability-fairness-bias, investigating-ableism-mt-conversation} has also shown that models imbibe harmful generalisations and stereotypes about people with disabilities. LLMs tend to associate mentions of disability with perceived negativity~\cite{hassan2021unpacking-ableist-intersectional}. They mirror many prejudices from the training dataset, subtly reinforcing many harmful assumptions about people with disabilities~\cite{disability-centred-llm-perspectives}. These baked-in stereotypes may lead to models discriminating against people who disclose a disability in the hiring process~\cite{impact-disability-fairness-bias}. They also result in overgeneralizations which cause people with disabilities to be misrepresented by these models. Although these are related to our work, they focus on studying disabilities and the prejudice associated with them in isolation. On the other hand, we focus primarily on the cross-study of how disabilities cause models to make biased presumptions about other attributes, such as gender, economic status, and education level.

% TODO: Find relevant papers
\subsection{Hallucinations and abstention} LLMs are known to assume stereotypes and often hallucinate or fabricate facts to justify their assumptions~\cite{Kotek2023GenderBA}.Wan et. al ~\cite{wan2023kellywarmpersonjoseph} introduces the term “hallucination bias”, where LLMs fabricate gendered traits not grounded in input, while Kamruzzaman et al.~\cite{kamruzzaman-etal-2024-investigating} discuss how experiments show that LLMS depict preferential descriptions, with elite Western affiliations being favoured. Previous research has explored ways to combat this through fine-tuning or prompting them to abstain from inferring in cases where there is lack of appropriate context ~\cite{yadkori2024mitigatingllmhallucinationsconformal, madhusudhan2024llmsknowanswerinvestigating}. However, it is noted that  even state-of-the-art LLMs like GPT-4 struggle with abstention, though strategic prompting, such as Chain-of-Thought, can significantly enhance this ability ~\cite{madhusudhan2024llmsknowanswerinvestigating}.

\subsection{Intersectionality of biases}

There has been limited analysis of how the intersection of multiple biases impacts a model’s perception of an individual. Previous works~\cite{cheng2023marked-personas-intersectional, hassan2021unpacking-ableist-intersectional, decoding-ableism-intersectional-llm, intersectional-stereotypes} have primarily examined how LLMs behave when presented with multiple marginalized identities. Notably,~\cite{decoding-ableism-intersectional-llm} focused on how disability interacts with other social categories. In contrast, our work investigates how disability cues lead models to make inferences about unrelated attributes.

Several datasets document harmful stereotypes in intersectional contexts. \cite{cheng2023marked-personas-intersectional} introduced a benchmark to probe identity-based behavior. \cite{intersectional-stereotypes} proposed a dataset capturing stereotype prevalence in three LLMs across intersectional groups. Building on~\cite{cao2022theory, cheng2023marked-personas-intersectional}, it used full-sentence prompts rather than individual words, enabling more complex stereotype analysis.

\cite{hassan2021unpacking-ableist-intersectional} examined ableist bias in BERT using a sentiment analysis task. They showed increased negative sentiment when disability was introduced but found minimal changes under intersectional conditions. Their approach was limited by a narrow verb set and overlapping identity categories. \cite{decoding-ableism-intersectional-llm} studied ableist bias in LLMs across multiple identity combinations using sentiment and social perception metrics. They found that while GPT-4 was less biased than GPT-3.5, bias persisted, especially in intersectional cases.

Some work has explored bias mitigation. \cite{correcting-underrepresentation-intersectional} addressed underrepresentation by inferring dropout rates across identity attributes from small, unbiased samples. \cite{mitigate-intersectional-diffusion} proposed a disentangled attention mechanism to reduce intersectional bias in diffusion models. However, both focus primarily on gender; disability intersections remain underexplored.

A significant limitation in current work in this area is the lack of work on how models perceive the correlation between different attributes or identities. Prior research on intersectional biases primarily served to analyze the biases and stereotypes that were perpetuated at the intersection of disabilities with other attributes, and largely left the correlation between them unstudied. Hence, in this paper, we attempt to analyze how models correlate disabilities with various attributes, such as gender, income, and locality.

\section{Methodology}
 While prior studies have consistently shown that LLMs exhibit systematic biases, including the reinforcement of societal stereotypes and skewed sentiment associations across demographic and occupational domains, this has rarely been examined specifically within the context of accessibility. Thus, this paper analyses the correlation between a model's bias towards people with disabilities and their other attributes, and whether models are more likely to make stereotypical assumptions in the case of people with disabilities.
 
  We do so by by querying the LLM  and prompting it to assign gender, economic, educational and cultural attributes to the user\footnote{Please note that many of these, while not truly binary attributes, are presented to the model as binary choices. We make this choice to maintain consistency across attributes and to further demonstrate the tendency of models to make assumptions and perpetuate such prejudices.}, asking this query for both cases where the user is assumed to have no disability and the case where the user is assumed to have a specific disability. We term the percentage of queries to which an LLM responds with a valid option as the response rate. We then compare overall response rates as well as biases towards one label in the attribute over the other.
  
  \subsection{Dataset Selection}
  For our experiments, we use the AccessEval dataset, which consists of paired queries in six real world business domains: Education, Finance, Healthcare, Hospitality, Media, and Technology. The pairs are as follows:

  \begin{itemize}
      \item A \textbf{Neutral Query (NQ)}, which does not reference any disability, and
      \item A corresponding \textbf{Disability Aware Query (DQ)}, which explicitly incorporates disability related context through placeholders for nine disability categories(for systemic evaluation) 
  \end{itemize}

   In this work, we consider the following disability types: Vision impairments, Hearing impairments, Speech impairments, Mobility impairments, Neurological disorders, Genetic and developmental disorders, Learning disorders, Sensory and cognitive disorders, and Mental and behavioral disorders.

  \subsection{Query Formation}
  For the purpose of determining correlations between biases and disability labels, we define five main attributes that we with for the LLM to evaluate the query and assign user labels on: Gender (with label pairs --- male, female), Socioeconomic Status (with label pairs --- Low income, High income), Geographic Location (with label pairs --- Urban, Rural), Educational Background (with label pairs --- Low, High) and Cultural Background(with label pairs --- Western, Non western).
  We then prompt the LLM to determine which label is more apt for the user for each of the five attributes based on the query asked. This is for all ten cases (one with the NQ and one for each of the 9 DQs).

  \subsection{Models}

  Since our aim is to investigate intersectional bias in SOTA LLMs, we chose a representative selection of LLMs covering a variety of sizes and architectures ---
  \begin{itemize}
      \item \textbf{Small ($\sim$3B)} --- Llama-3.2-3B-Instruct~\cite{llama3}, Phi-4-Mini-Instruct~\cite{phi4mini}, and Qwen-2.5-3B-Instruct~\cite{qwen2.5}
      \item \textbf{Medium ($\sim$8B)} --- Llama-3.1-8B-Instruct~\cite{llama3}, Ministral-8B-Instruct~\cite{ministral}, and Qwen-2.5-7B-Instruct~\cite{qwen2.5}
      \item \textbf{Large ($\sim$70B)} --- Llama-3.3-70B-Instruct~\cite{llama3} and Qwen-2.5-72B-Instruct~\cite{qwen2.5}
  \end{itemize}
  
  This selection enables a systematic analysis of how intersectional bias manifests across model scales and architectural design choices, facilitating insights into the dynamics of disability-related intersectional bias in contemporary instruction-tuned LLMs.

\subsection{Do LLMs respond to Biased Attributes?}

\begin{figure*}
  \centering
  \begin{subfigure}{0.49\linewidth}
    \includegraphics[width=\textwidth]{ICCV2025-Author-Kit-Feb/fig/rq1_neutral.png}
    \caption{Average response rate across attributes on neutral queries.}
    \label{fig:short-a}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.49\linewidth}
    \includegraphics[width=\linewidth]{ICCV2025-Author-Kit-Feb/fig/rq1_disability.png}
    \caption{Average response rate across attributes on disability queries.}
  \end{subfigure}
  \caption{Comparison of the response rate of models on neutral and average of disability queries. Models with the same color have similar parameter counts.}
  \label{fig:rq1-response-rate}
\end{figure*}

As seen in Figure~\ref{fig:rq1-response-rate}, the average response rate in the neutral scenario averaged across all attributes is 58.6\%, with significant variation between models. Phi-4 shows the lowest response bias i.e. highest abstention rate on average compared to all other models. This remains consistent in both disability and non-disability contexts. It has a response rate of 15\% in the neutral scenario and 13\% on average across disabilities. Qwen 72B, on the other hand, has the highest response rate, barely abstaining from answering queries in either scenario. It has a response rate of 97\% in a disability context and 94\% in a neutral context. We see that overall, the response rate remains relatively unchanged both in the neutral scenario and in the average disability scenario, with a maximum change of 4\% displayed by Qwen 7B. The only exception to this is Llama 3.3 with an increase of 12\% response rate in the average disability scenario. There is an overall average increase of 1.5\% on disability queries as compared to neutral queries, however, this is primarily driven by the outlier increase in Llama 3.3. Excluding Llama 3.3, the average increase or decrease in response rates in the disability scenario is 0\%.

Hence, we see that the presence or absence of a disability, on average, \textbf{does not have any noticeable effect} on the response rate of a model. This also shows the limitations of current techniques in the context of abstaining from answering sensitive queries, especially when it comes to disabilities.

\begin{table}
  \centering
  \resizebox{\linewidth}{!}{%
    \begin{tabular}{@{}lcc@{}}
      \toprule
      Model Size & Neutral Scenario (\%) & Disability Scenario (\%) \\
      \midrule
      Small (3--3.8B) & 48.9 & 49.1 \\
      Medium (7--8B) & 53.7 & 53.3 \\
      Large (70B+) & 81.9 & 89.9 \\
      \bottomrule
    \end{tabular}%
  }
  \caption{Average response rates by model size in neutral and disability scenarios.}
  \label{tab:response-rates}
\end{table}

We also observe in table~\ref{tab:response-rates} that increasing model size also \textbf{increases its response rate.} Previous works have shown that larger models are seen to have better performance by both qualitative and quantitative metrics, but we observe that this is not the case with response bias. Response bias remains prevalent in larger models. As the table shows, the average response rate of models having on the order of 70B parameters is 81.9\% in the neutral scenario and 89.9\% in the disability scenario, whereas that of small models is only 48.9\% in the neutral scenario and 49.1\% in the disability scenario. This suggests that while larger models are better at generating fluent and relevant responses, they may also be less cautious, making them more likely to answer biased or inappropriate questions unless stronger safety measures are in place.

\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{ICCV2025-Author-Kit-Feb/fig/rq1_radar.png}
  \caption{Average response rate for each attribute on neutral queries.}
  \label{fig:rq1-radar}
\end{figure}

As we observed in figure~\ref{fig:rq1-response-rate}, response rate is not significantly impacted by presence or absence of a disability. It is also not affected by the specific disability type, as we discuss in our supplementary material. However, figure~\ref{fig:rq1-radar} shows that attributes have a very noticeable impact on the response rate. Further, the response graphs vary visibly between models. For instance, the 70B models tend to respond to all questions equally regardless of attribute. Ministral primarily responds only to questions on education, at a response rate of 90.2\%, while Llama 3.2 3B responds relatively evenly to all queries except gender, where it strongly abstains. We observe that economic status has the lowest response rate across models on average of 40.3\%, closely followed by gender at 43.8\%. Meanwhile, education has by far the highest response rate of 71.7\%. These findings suggest that models are not uniformly sensitive to demographic attributes, as certain topics like education prompt high response rates, while others like gender or economic status elicit more caution or uncertainty. This uneven responsiveness hints at implicit prioritizations during training, in terms of which attributes are considered sensitive and how safety behaviors are calibrated.

\subsubsection{Response Rate by Disability Type}

\begin{figure}[h]
  \centering
  \includegraphics[width=\linewidth]{ICCV2025-Author-Kit-Feb/fig/rq2.1_avg.png}
  \caption{Average response rate for each disability type mentioned in the query. Neutral represents no disability mentioned.}
  \label{fig:rq2.1-avg}
\end{figure}

Figure~\ref{fig:rq2.1-avg} shows the average response rate for each model across disability types. While the overall response rate is relatively stable within each model, subtle but consistent differences emerge across specific attributes. Notably, as observed earlier, models tend to respond at almost equal rates whether the query contains a mention of disability or not, with a slight change in response rate observed for certain disability-related queries. 

Small models show more noticeable trends in terms of having greater variance in response rates based on disability type. For instance, Qwen 7B responds at a noticeably higher rate to queries where genetic and developmental disorders are mentioned. In contrast, larger models like Llama 3.3 70B and Mistral 8B maintain higher and more consistent response rates across all categories. We also notice a visible difference between model families, with all three Llama models generally having a response rate over 70\%, while in the Qwen model family, only the largest model, 72B, shows a response rate above 40\%. This trend is observed across disability types.

This suggests that model size and architecture all play a role in robustness to disability-related prompts, potentially reflecting differences in training scale, alignment strategies, or exposure to diverse linguistic representations of disability.

\subsection{LLM bias in a disability scenario}
% RQ3.1 Figures
\begin{figure*}
\centering
  \begin{subfigure}{0.49\linewidth}
    \includegraphics[width=\textwidth]{fig/rq3/rq3.1_gender.png}
    \caption{Gender}
    \label{fig:rq3.1-attributes-gender}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.49\linewidth}
    \includegraphics[width=\textwidth]{fig/rq3/rq3.1_income.png}
    \caption{Income}
    \label{fig:rq3.1-attributes-income}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.49\linewidth}
    \includegraphics[width=\textwidth]{fig/rq3/rq3.1_western.png}
    \caption{Culture}
    \label{fig:rq3.1-attributes-culture}
  \end{subfigure}

  \vspace{0.5em}

  \begin{subfigure}{0.49\linewidth}
    \includegraphics[width=\textwidth]{fig/rq3/rq3.1_locality.png}
    \caption{Locality}
    \label{fig:rq3.1-attributes-locality}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.49\linewidth}
    \includegraphics[width=\textwidth]{fig/rq3/rq3.1_education.png}
    \caption{Education}
    \label{fig:rq3.1-attributes-education}
  \end{subfigure}

  \caption{Model bias by attribute for various disability types. Note the significant variations in bias based on disability type.}
  \label{fig:rq3.1-attributes}
\end{figure*}

% RQ3.2 Figures
\begin{figure*}
\centering
  \begin{subfigure}{0.49\linewidth}
    \includegraphics[width=\textwidth]{fig/rq3/rq3.2_gender.png}
    \caption{Gender}
    \label{fig:rq3.2-attributes-gender}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.49\linewidth}
    \includegraphics[width=\textwidth]{fig/rq3/rq3.2_income.png}
    \caption{Income}
    \label{fig:rq3.2-attributes-income}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.49\linewidth}
    \includegraphics[width=\textwidth]{fig/rq3/rq3.2_western.png}
    \caption{Culture}
    \label{fig:rq3.2-attributes-culture}
  \end{subfigure}

  \vspace{0.5em}

  \begin{subfigure}{0.49\linewidth}
    \includegraphics[width=\textwidth]{fig/rq3/rq3.2_locality.png}
    \caption{Locality}
    \label{fig:rq3.2-attributes-locality}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.49\linewidth}
    \includegraphics[width=\textwidth]{fig/rq3/rq3.2_education.png}
    \caption{Education}
    \label{fig:rq3.2-attributes-education}
  \end{subfigure}

  \caption{Model biases by attribute for different question domains. Notice the variance in bias across domains.}
  \label{fig:rq3.2-attributes}
\end{figure*}
As visible in figure~\ref{fig:rq3.1-attributes-gender}, there is a general male bias irrespective of the existence or type of disability though not nearly as strong a preference as is there in other attribute pairs. However, it is also visible that there is a significant variance in model responses, based on both the mention of a disability, as well as the type of disability mentioned. The models depict a strong tendency to associate neutrality (lack of disabilities) with the male gender. Addtionally there was a smaller, but still noticeable spike in assumptions of male gender in the case of learning disorders, neurological disorders and speech impairments. Conversely, while disabilities in general are clearly associated with the female gender there is a distinct spike when it comes to sensory and cognitive disorders. The model's consistent association of male gender with “no disability” aligns with the sociological concept of male default normativity. The spike toward male gender predictions for learning disorders, neurological disorders, and speech impairments may reflect gendered health biases that perceive such disabilities as more typical in boys (e.g., ADHD, autism) - consistent with psychological research showing higher male diagnosis rates and stronger stereotypes linking neurological differences with males, while the overall trend reflects an intersectional stereotype: linking disability with dependence/vulnerability, and further associating that with femininity.

Another interesting observation is made with respect to the responses of models with respect to model size. While LLama moves from a strong female bias towards people with disabilities towards an almost 50-50 response (demonstrating possible randomisation in larger models) with an increase in model size, Qwen 3B has a low response rate and an almost 100\% male bias while Qwen 72 B has a much higher response rate and has an almost 100 percent female response rate.

With respect to~\ref{fig:rq3.1-attributes-income}, all models except LLama 3B depict a strong general bias toward predicting a higher economical class. This is further exacerbated in the case of NQs, leading us to assume that it associates disabilities in general with lower income classes. Due to this, there is less of a trend seen in models with respect to individual disability types with respect to economic status, especially since the models tend to predict high income irrespective of whether a disability is present in the query. The models do, however, show relative associations of low income responses with mobility impairments, genetic and developmental disorders, mental health and behavioral disorders, and speech impairments. Models with lower response rates also demonstrate relatively higher association of lower income with sensory and cognitive disabilities. However, models are much less likely to associate neurological disorders and hearing disorders with lower income. The relative association of certain disability types with poverty reflects real-world ableist economic stereotypes, where visible or developmental disabilities are linked to dependence or reduced opportunity. Some disability types like hearing loss or neurological conditions escape this association, reflecting asymmetric bias and underscoring how models may absorb cultural myths around "competent" versus "dependent" disabilities.

In the case of attributes regarding Culture, Educational Levels and Localities, the model overwhelmingly assumes the association of any query irrespective of disability with Western, Urban and  High Education as observed in figures~\ref{fig:rq3.1-attributes-culture}, \ref{fig:rq3.1-attributes-education}, and \ref{fig:rq3.1-attributes-locality}. This is demonstrates the models' bias, as well as their willingness to assume one label over the other in attributes that are not traditionally considered sensitive. In the case of Culture (\ref{fig:rq3.1-attributes-culture}), we can see that Ministral 8B and Qwen 2.5 3B tend to relatively associate Genetic and Developmental Disorders, Mobility Impairments and Sensory and Cognitive Disorders with non-western communities. Additionally, they also associate almost 100\% of neutral queries with western communities. However due to the highly skewed nature of the results, commenting on this in an accessibility context becomes difficult.

 In the case of Locality (\ref{fig:rq3.1-attributes-locality}), the models assume that the user is from an urban region with almost 100\% likelihood, thus making disability-specific investigations irrelevant. The models' responses in the case of Education(\ref{fig:rq3.1-attributes-education}) appear to be more significant, with almost all models having a near 100\% likelihood of assuming high education in the case of neutral queries. Learning disabilities and Genetic and Developmental disorders on the other hand, seem to have a relative dip, pointing to their relative association with lower education. The models also tend to assume a stronger likelihood of Sensory and Cognitive disabilities in highly educated people. However, the overall symmetry of the graph points to the net bias of the model towards higher education outweighing any disability specific bias.

 The existence of a general trend among models enables us to examine the overall behaviour displayed with respect to each disability. Another way we examine it is through the lens of business domains. 

 Figure (\ref{fig:rq3.2-attributes}) depicts that the models tend to show common spikes with respect to business domains, irrespective of the presence of a disorder or the specific type of disorder mentioned. In the case of Gender(\ref{fig:rq3.2-attributes-gender}), All NQs and DQs show a distinct association of the male gender with Technology, Healthcare and Finance, while strongly associating Education and Hospitality with the female Gender.

 In the case of Income(\ref{fig:rq3.2-attributes-income}) the models respond with 'low income less than 20 \% of the time in the case of every business domain except Finance, where the percent of low income responses doubles. 
 
  In the case of Culture(\ref{fig:rq3.2-attributes-culture}) and Locality(\ref{fig:rq3.2-attributes-locality}) the models respond with western, and urban respectively nearly 100\% of the time displaying a common bias irrespective of disability or business domain. In the case  of Education Level(\ref{fig:rq3.2-attributes-education}) the graph is almost symmetrical, although models do notably assume a lower education level for questions posed by people with learning disabilities in finance. However the overall symmetry in the graph tends to represent a net bias towards answers that assume every user has a high education level.

  All in all, it is clear that domain specific biases have a tendency to influence model answers more than disability specific biases, though the strength of association varies based on the existence of a disability and the disability type in a manner similar to that discussed in figure (\ref{fig:rq3.1-attributes}).

\section{Conclusion}
We have provided the first systematic evaluation of how self-declared disability contexts affect demographic inference and stereotype amplification in leading large language models. Across nine disability categories and five demographic attributes, we found that overall response rates change minimally ($\approx$1.5\% on average). Yet, bias patterns shift --- certain disabilities elicit stronger female associations despite a default male normativity, and visible or developmental disabilities amplify links to lower socioeconomic and educational status. Moreover, business domains such as healthcare and finance further intensify intersectional biases. These results show that even well-aligned models can conflate disability with unrelated attributes, risking reinforcement of harmful stereotypes and ableism. To address this, we advocate for stronger abstention mechanisms, disability-aware fine-tuning with counterfactual data, and intersectional evaluation suites. Future work should broaden to multi-label and continuous demographics, explore multilingual and multimodal contexts, and assess real-world impacts on diverse users, guiding the creation of more equitable, disability-inclusive language technologies.

\section{Limitations}
Our analysis covers a carefully curated set of English-only models, controlled template prompts specifically designed for demographic inference, and nine broad disability categories, which may not fully capture the rich variability of real-world conversations, multiple disabilities occurring simultaneously, or the full spectrum of diverse non-English cultural frameworks. Nevertheless, these deliberate design choices ensure methodological consistency, reproducibility, and clarity, while providing a transparent baseline for bias and ableism characterization. Future work should extend to more recent or multimodal model architectures, incorporate even finer-grained and intersecting disability labels, explore naturalistic multi-turn dialogues and realistic downstream applications at scale, and involve a broader selection of languages, dialects, and regional contexts to deepen our understanding of how ableism emerges in language models and to reinforce effective mitigation strategies, ultimately guiding the development of more universally inclusive and disability-aware systems.  




%% ORIGINAL CONCLUSION, USE FOR REFERENCE
% \section{Conclusion}
% In this work, we have presented the first systematic analysis of how self-declared disability contexts influence demographic inference and stereotype amplification in state-of-the-art large language models. Through controlled experiments across nine distinct impairment categories and five key user attributes (gender, socioeconomic status, geographic location, education level, and cultural background), we demonstrated that:
% \begin{itemize}
%   \item \textbf{Response rate remains largely unchanged} when disability is mentioned, with only a marginal overall increase in response rates (1.5\% on average) and model-specific variations driven by scale and architecture.
%   \item \textbf{Bias patterns shift in disability contexts}: models exhibit stronger male default normativity in neutral queries but show even higher female associations for certain disabilities (e.g., sensory and cognitive disorders), reflecting real-world diagnostic and societal stereotypes.
%   \item \textbf{Economic and educational stereotypes are exacerbated}: models disproportionately link visible or developmental impairments (e.g., mobility, learning disorders) with low socioeconomic or lower educational status, while maintaining strong default associations of high income, high education, Western culture, and urban locality in most scenarios.
%   \item \textbf{Intersectional biases vary by domain}: business contexts such as healthcare and finance further amplify certain attribute predictions, underscoring the need for domain-aware bias audits.
% \end{itemize}

% These findings highlight that even models with advanced alignment and safety training can unknowingly conflate disability with other sensitive attributes, potentially reinforcing harmful stereotypes and reducing accessibility for people with disabilities. To mitigate these risks, we recommend:
% \begin{enumerate}
%   \item \textbf{Improved abstention mechanisms} --- Designing models to exhibit stronger refusal behavior when insufficient evidence exists for demographic inference, particularly in sensitive contexts.
%   \item \textbf{Disability-aware fine-tuning} --- Inclusion of disability-centered corpora and counterfactual augmentation to decouple impairment labels from unrelated attributes.
%   \item \textbf{Intersectional evaluation suites} --- Development of benchmark datasets that systematically combine disability with other demographic dimensions and application domains.
%   % \item \textbf{User-centric interface design} --- Transparent explanations and override options that allow users to correct or opt out of inferred assumptions.
% \end{enumerate}

% Future work should extend beyond binary attribute pairs to multi-label and continuous demographic spectra, explore mitigation strategies in multilingual and multimodal settings, and evaluate real-world impacts on diverse user populations. By deepening our understanding of disability-related intersectional bias, we can guide the development of more equitable and inclusive language technologies.

% % \medskip
% % \noindent\textbf{Acknowledgments.} We thank the anonymous reviewers for their detailed feedback, and our colleagues in the Accessibility and Fairness groups for valuable discussions on methodology and ethics.

% \section{Limitations}
% While our study provides a comprehensive first look at how self‐declared disability contexts interact with demographic inference in large language models, there are several important limitations to note:
% \begin{itemize}
%   \item \textbf{Model selection and versions.} We evaluated a representative but finite set of commercial and research models available at the time of writing. Future releases or alternative architectures (e.g., very large multimodal systems) may exhibit different bias patterns.
%   \item \textbf{Prompt design and framing.} Our controlled prompts target only direct demographic inference tasks; real‐world user queries are more varied in style, phrasing, and context, which may affect both response behavior and bias manifestation.
%   \item \textbf{Disability scope.} We focus on nine broad impairment categories and self‐declared labels; more granular or comorbid disability types (e.g., dual sensory loss, mental health conditions) and intersection with other identities (e.g., race, age) remain unexplored.
%   \item \textbf{Synthetic evaluation setting.} By design, our benchmarks depend on template‐based prompts rather than conversational logs or downstream applications, limiting ecological validity for dynamic, multi‐turn interactions.
%   \item \textbf{Cultural and linguistic bias.} All experiments are conducted in English and reflect Western diagnostic norms; findings may not generalize to non‐English languages or cultural frameworks of disability.
%   % \item \textbf{Metric limitations.} We measure response rate and attribute association via proxy metrics (e.g., top‐k word associations), which capture only first‐order biases and may not reflect subtler or latent stereotyping.
% \end{itemize}

==> sec/conclusion.tex <==
\section{Conclusion}
We have provided the first systematic evaluation of how self-declared disability contexts affect demographic inference and stereotype amplification in leading large language models. Across nine disability categories and five demographic attributes, we found that overall response rates change minimally ($\approx$1.5\% on average). Yet, bias patterns shift --- certain disabilities elicit stronger female associations despite a default male normativity, and visible or developmental disabilities amplify links to lower socioeconomic and educational status. Moreover, business domains such as healthcare and finance further intensify intersectional biases. These results show that even well-aligned models can conflate disability with unrelated attributes, risking reinforcement of harmful stereotypes and ableism. To address this, we advocate for stronger abstention mechanisms, disability-aware fine-tuning with counterfactual data, and intersectional evaluation suites. Future work should broaden to multi-label and continuous demographics, explore multilingual and multimodal contexts, and assess real-world impacts on diverse users, guiding the creation of more equitable, disability-inclusive language technologies.

\section{Limitations}
Our analysis covers a carefully curated set of English-only models, controlled template prompts specifically designed for demographic inference, and nine broad disability categories, which may not fully capture the rich variability of real-world conversations, multiple disabilities occurring simultaneously, or the full spectrum of diverse non-English cultural frameworks. Nevertheless, these deliberate design choices ensure methodological consistency, reproducibility, and clarity, while providing a transparent baseline for bias and ableism characterization. Future work should extend to more recent or multimodal model architectures, incorporate even finer-grained and intersecting disability labels, explore naturalistic multi-turn dialogues and realistic downstream applications at scale, and involve a broader selection of languages, dialects, and regional contexts to deepen our understanding of how ableism emerges in language models and to reinforce effective mitigation strategies, ultimately guiding the development of more universally inclusive and disability-aware systems.  




%% ORIGINAL CONCLUSION, USE FOR REFERENCE
% \section{Conclusion}
% In this work, we have presented the first systematic analysis of how self-declared disability contexts influence demographic inference and stereotype amplification in state-of-the-art large language models. Through controlled experiments across nine distinct impairment categories and five key user attributes (gender, socioeconomic status, geographic location, education level, and cultural background), we demonstrated that:
% \begin{itemize}
%   \item \textbf{Response rate remains largely unchanged} when disability is mentioned, with only a marginal overall increase in response rates (1.5\% on average) and model-specific variations driven by scale and architecture.
%   \item \textbf{Bias patterns shift in disability contexts}: models exhibit stronger male default normativity in neutral queries but show even higher female associations for certain disabilities (e.g., sensory and cognitive disorders), reflecting real-world diagnostic and societal stereotypes.
%   \item \textbf{Economic and educational stereotypes are exacerbated}: models disproportionately link visible or developmental impairments (e.g., mobility, learning disorders) with low socioeconomic or lower educational status, while maintaining strong default associations of high income, high education, Western culture, and urban locality in most scenarios.
%   \item \textbf{Intersectional biases vary by domain}: business contexts such as healthcare and finance further amplify certain attribute predictions, underscoring the need for domain-aware bias audits.
% \end{itemize}

% These findings highlight that even models with advanced alignment and safety training can unknowingly conflate disability with other sensitive attributes, potentially reinforcing harmful stereotypes and reducing accessibility for people with disabilities. To mitigate these risks, we recommend:
% \begin{enumerate}
%   \item \textbf{Improved abstention mechanisms} --- Designing models to exhibit stronger refusal behavior when insufficient evidence exists for demographic inference, particularly in sensitive contexts.
%   \item \textbf{Disability-aware fine-tuning} --- Inclusion of disability-centered corpora and counterfactual augmentation to decouple impairment labels from unrelated attributes.
%   \item \textbf{Intersectional evaluation suites} --- Development of benchmark datasets that systematically combine disability with other demographic dimensions and application domains.
%   % \item \textbf{User-centric interface design} --- Transparent explanations and override options that allow users to correct or opt out of inferred assumptions.
% \end{enumerate}

% Future work should extend beyond binary attribute pairs to multi-label and continuous demographic spectra, explore mitigation strategies in multilingual and multimodal settings, and evaluate real-world impacts on diverse user populations. By deepening our understanding of disability-related intersectional bias, we can guide the development of more equitable and inclusive language technologies.

% % \medskip
% % \noindent\textbf{Acknowledgments.} We thank the anonymous reviewers for their detailed feedback, and our colleagues in the Accessibility and Fairness groups for valuable discussions on methodology and ethics.

% \section{Limitations}
% While our study provides a comprehensive first look at how self‐declared disability contexts interact with demographic inference in large language models, there are several important limitations to note:
% \begin{itemize}
%   \item \textbf{Model selection and versions.} We evaluated a representative but finite set of commercial and research models available at the time of writing. Future releases or alternative architectures (e.g., very large multimodal systems) may exhibit different bias patterns.
%   \item \textbf{Prompt design and framing.} Our controlled prompts target only direct demographic inference tasks; real‐world user queries are more varied in style, phrasing, and context, which may affect both response behavior and bias manifestation.
%   \item \textbf{Disability scope.} We focus on nine broad impairment categories and self‐declared labels; more granular or comorbid disability types (e.g., dual sensory loss, mental health conditions) and intersection with other identities (e.g., race, age) remain unexplored.
%   \item \textbf{Synthetic evaluation setting.} By design, our benchmarks depend on template‐based prompts rather than conversational logs or downstream applications, limiting ecological validity for dynamic, multi‐turn interactions.
%   \item \textbf{Cultural and linguistic bias.} All experiments are conducted in English and reflect Western diagnostic norms; findings may not generalize to non‐English languages or cultural frameworks of disability.
%   % \item \textbf{Metric limitations.} We measure response rate and attribute association via proxy metrics (e.g., top‐k word associations), which capture only first‐order biases and may not reflect subtler or latent stereotyping.
% \end{itemize}


==> sec/revised_content.tex <==
\begin{abstract}
Large Language Models (LLMs) routinely make tacit assumptions about a user’s demographic background - such as gender, socioeconomic status, or education level - based solely on the phrasing and topical content of the user’s query. These hidden inferences can introduce bias even when no explicit personal information is provided. While automated demographic guessing has been extensively examined, the role of disability cues in shaping such inferences remains largely unexplored.

In this study, we investigate how explicit self‑disclosure of disability within a query reshapes the demographic assumptions made by state‑of‑the‑art LLMs. Using a controlled evaluation that spans nine disability categories and five core demographic attributes, we analyze both overall response rates and the shifts in predicted attribute distributions. Our results reveal that disability cues frequently re‑align model behavior, often reinforcing ableist stereotypes - for example, linking sensory‑processing disorders with lower income or associating learning disabilities with non‑Western identities. These effects become more pronounced in domain‑specific contexts such as healthcare and finance.

Our findings emphasize the urgent need for intersectional fairness audits that treat disability as a first‑class dimension and highlight the importance of model‑design choices that discourage overconfident demographic inference from limited user context.
\end{abstract}

\section{Introduction}
\label{sec\:intro}

Large Language Models (LLMs) increasingly drive applications that personalize content, improve accessibility, and deliver context‑aware support\~\cite{brown2020languagemodelsfewshotlearners,openai2024gpt4technicalreport,Radford2018ImprovingLU}. However, these same models can infer sensitive demographic information - including gender, socioeconomic status, geographic location, and education level - from user queries even when explicit identifiers are absent. The presence of disability‑related language may amplify or redirect these inferences, producing intersectional biases that disproportionately impact people with disabilities\~\cite{Caliskan\_2017, Gallegos2023BiasAF, Hall2022ASS, Kotek2023GenderBA}.

Recent work\~\cite{cheng2023marked-personas-intersectional,decoding-ableism-intersectional-llm, mitigate-intersectional-diffusion} shows that LLMs frequently associate disability terms with negative sentiment or deficit‑oriented frames, thereby perpetuating societal stigma. Unlike gender‑ or race‑related bias - where richer benchmarking infrastructure exists - disability bias remains under‑resourced, complicating detection and mitigation. Understanding how representational and stereotype bias amplification manifests in disability contexts is therefore an overdue research priority.

Current mitigation strategies often rely on guardrails that prevent a model from releasing sensitive information, but these do not address the root problem: the model’s internal beliefs\~\cite{yuan2024rigorllmresilientguardrailslarge}. When an LLM is prompted to infer an attribute for which it lacks sufficient evidence, a desirable behavior is to refuse. Yet we demonstrate that state‑of‑the‑art models frequently respond regardless, reflecting learned biases.\~\cite{yadkori2024mitigatingllmhallucinationsconformal}.

This paper systematically examines how disability cues influence demographic inference, aiming to highlight bias patterns, surface blind spots, and inform ethical model deployment.

%-------------------------------------------------------------------------

The key contributions of this paper are as follows:
\begin{enumerate}
\item We demonstrate that state‑of‑the‑art LLMs frequently respond to demographic inference prompts in both neutral and disability‑aware scenarios.
\item We show that these responses are systematically biased. Moreover, bias patterns vary markedly between neutral and disability‑specific contexts and interact with business domains and disability types.
\end{enumerate}

\section{Background and Related Works}

\subsection{Bias in LLMs}
LLMs achieve impressive performance across many NLP tasks, yet they remain vulnerable to representational bias and stereotyping. Prior studies show that LLMs absorb and amplify harmful societal biases - particularly those tied to gender, race, religion, and health - across contextual embeddings and generated text\~\cite{Caliskan\_2017, Gallegos2023BiasAF, Kumar2022LanguageGM}. These models often mirror imbalances present in their training corpora rather than reflecting equitable associations\~\cite{Hall2022ASS, Nadeem2020StereoSetMS, Kotek2023GenderBA}. Although gender and race have been extensively benchmarked, emerging work highlights bias against people with disabilities.

\subsection{Disability bias}
Research indicates that LLMs can embody harmful generalizations about people with disabilities\~\cite{disability-centred-llm-perspectives, impact-disability-fairness-bias, investigating-ableism-mt-conversation}. Models frequently associate disability mentions with negative sentiment\~\cite{hassan2021unpacking-ableist-intersectional} and perpetuate ableist stereotypes\~\cite{disability-centred-llm-perspectives}. Such patterns risk discrimination—for instance, against job applicants who disclose disabilities\~\cite{impact-disability-fairness-bias}. While related studies investigate disability bias in isolation, we focus on how disabilities prompt models to infer other attributes (e.g., gender, income, education).

\subsection{Hallucinations and abstention}
LLMs are prone to hallucinating facts or reinforcing stereotypes when context is insufficient\~\cite{Kotek2023GenderBA}. Wan\~\emph{et al.}~~\cite{wan2023kellywarmpersonjoseph} introduce “hallucination bias,” where models fabricate gendered traits; Kamruzzaman~~\emph{et al.}~~\cite{kamruzzaman-etal-2024-investigating} find a preference for elite Western affiliations. Although strategic prompting improves abstention~~\cite{madhusudhan2024llmsknowanswerinvestigating}, even GPT‑4 often answers when it should refuse.

\subsection{Intersectionality of biases}
Earlier work on intersectionality examines how LLMs respond when multiple marginalized identities intersect\~\cite{cheng2023marked-personas-intersectional,hassan2021unpacking-ableist-intersectional,decoding-ableism-intersectional-llm,intersectional-stereotypes}. For example, \cite{decoding-ableism-intersectional-llm} shows that GPT‑4 is less biased than GPT‑3.5 but bias persists, especially in intersectional contexts. However, little research explores how disability cues lead models to infer unrelated attributes—our focus here.

\section{Methodology}
While prior studies demonstrate systemic biases in LLMs, few examine the accessibility context. We analyze whether disability cues increase stereotypical assumptions about unrelated demographic attributes.

We query each model with prompts that ask it to assign gender, economic status, education level, geographic locality, and cultural background to the user. We measure the \emph{response rate}—the fraction of prompts where the model selects a label rather than refusing—comparing the neutral case (no disability mentioned) with each disability type.

\subsection{Dataset Selection}
We use the dataset introduced by~\cite{anonymous2025}, which pairs six domain‑specific queries (Education, Finance, Healthcare, Hospitality, Media, Technology) in two forms:
\begin{itemize}
\item \textbf{Neutral Query (NQ):} No disability is mentioned.
\item \textbf{Disability‑Aware Query (DQ):} The same query explicitly mentions one of nine disability categories.
\end{itemize}
Disability types include: Vision, Hearing, Speech, Mobility, Neurological, Genetic and Developmental, Learning, Sensory and Cognitive, and Mental and Behavioral.

\subsection{Query Formation}
We evaluate five binary attributes: Gender (male/female), Socioeconomic Status (low/high income), Geographic Location (urban/rural), Educational Background (low/high), and Cultural Background (Western/non‑Western). For each query variant (one NQ + nine DQs), we prompt the model to select the most plausible label for each attribute.

\subsection{Models}
To probe bias across scales, we evaluate:
\begin{itemize}
\item \textbf{Small ($\sim$3B)} - Llama‑3.2‑3B‑Instruct\~\cite{llama3}, Phi‑4‑Mini‑Instruct\~\cite{phi4mini}, Qwen‑2.5‑3B‑Instruct\~\cite{qwen2.5}
\item \textbf{Medium ($\sim$8B)} - Llama‑3.1‑8B‑Instruct\~\cite{llama3}, Mistral‑8B‑Instruct\~\cite{ministral}, Qwen‑2.5‑7B‑Instruct\~\cite{qwen2.5}
\item \textbf{Large ($\sim$70B)} - Llama‑3.3‑70B‑Instruct\~\cite{llama3}, Qwen‑2.5‑72B‑Instruct\~\cite{qwen2.5}
\end{itemize}
This lineup enables systematic analysis of how bias evolves with model size and architecture.

\section{Results and Discussion}
\subsection{Do LLMs respond to biased attributes?}

Our analysis (Figure\~\ref{fig\:rq1-response-rate}) shows that the mean response rate in the neutral scenario is 58.6\%, with substantial model‑to‑model variance. Phi‑4 displays the lowest response tendency (highest abstention), while Qwen‑72B almost never refuses. Overall, disability cues shift response rates by only $\approx$1.5\% (driven mainly by Llama‑3.3), indicating that simply mentioning disability does not trigger higher abstention.

Table\~\ref{tab\:response-rates} further reveals a size trend: larger models respond more, contrary to the expectation that greater capacity yields safer behavior. The 70B‑parameter class exceeds 80% response rate in both neutral and disability contexts, compared with $<55\%$ for small models.

Figure\~\ref{fig\:rq1-radar} confirms that response rates vary more by attribute than by disability context. Economic status elicits the greatest caution (40.3\%), whereas education prompts the highest response (71.7\%). This suggests implicit prioritization in safety training.

\subsubsection{Response rate by disability type}

Figure\~\ref{fig\:rq2.1-avg} indicates that model family and scale, rather than disability type, primarily drive response variance. Nonetheless, some small models show elevated response rates for genetic/developmental disorders, hinting at asymmetric safety tuning.

\subsection{LLM bias in a disability scenario}
\[Figures and captions unchanged; see PDF.]

Figure\~\ref{fig\:rq3.1-attributes-gender} reveals a default male normativity for neutral queries, yet female associations spike for certain disabilities—particularly sensory and cognitive disorders—echoing sociological mappings of vulnerability to femininity. Llama models shift toward parity with scale, whereas Qwen exhibits near‑polar biases between 3B and 72B variants, suggesting divergent alignment strategies.

Figure\~\ref{fig\:rq3.1-attributes-income} shows that most models predict high income by default; nevertheless, visible or developmental disabilities (mobility, learning) nudge predictions toward low income, mirroring ableist economic stereotypes. Cultural, locality, and education attributes display overwhelming Western, urban, and high‑education assumptions (Figures\~\ref{fig\:rq3.1-attributes-culture}–\ref{fig\:rq3.1-attributes-education}), indicating that these attributes are not treated as sensitive during alignment.

Domain analysis (Figure\~\ref{fig\:rq3.2-attributes}) finds consistent spikes: male‑gender predictions for technology, healthcare, and finance; female predictions for education and hospitality; double the low‑income rate in finance queries; and near‑universal Western/urban assumptions. Disability cues modulate but do not override these domain‑driven stereotypes.

\section{Conclusion}
We present the first systematic study of how explicit disability cues influence demographic inference in leading LLMs. Although average response rates change minimally, bias patterns shift: certain disabilities amplify female or low‑income associations, and business domains intensify intersectional effects. Our findings underscore that well‑aligned models can still entangle disability with unrelated attributes, risking ableist stereotyping.

We advocate for (1) stronger abstention mechanisms, (2) disability‑aware fine‑tuning with counterfactual augmentations, and (3) intersectional evaluation suites that treat disability as a core dimension. Future work should extend to multilingual and multimodal contexts, continuous demographics, and real‑world impact assessments.

\section{Limitations}
Our study evaluates a curated set of English‑only models, template‑based prompts, and nine disability categories. This design ensures reproducibility but limits ecological validity. Future research should explore newer architectures, finer‑grained and co‑occurring disabilities, multi‑turn dialogue, and diverse languages to deepen understanding and mitigation of ableism in language technologies.

